Geometric Median (GM) Matching for Robust Data Pruning

Large-scale data collections in the wild, are invariably noisy. Thus developing data pruning strategies that remain robust even in the presence of corruption is critical in practice. In this work, we propose Geometric Median ($\gm$) Matching -- a herding style greedy algorithm that yields a $k$-subset such that the mean of the subset approximates the geometric median of the (potentially) noisy dataset. Theoretically, we show that $\gm$ Matching enjoys an improved $\gO(1/k)$ scaling over $\gO(1/\sqrt{k})$ scaling of uniform sampling; while achieving {\bf optimal breakdown point} of {\bf 1/2} even under {\bf arbitrary} corruption. Extensive experiments across several popular deep learning benchmarks indicate that $\gm$ Matching consistently improves over prior state-of-the-art; the gains become more profound at high rates of corruption and aggressive pruning rates; making $\gm$ Matching a strong baseline for future research in robust data pruning.

==> ICLR-2025/main-paper/abstract.tex <==
Data pruning, the combinatorial task of selecting a small and informative subset from a large dataset, is crucial for mitigating the enormous computational costs associated with training data-hungry modern deep learning models at scale. Since large-scale data collections are invariably noisy, developing data pruning strategies that remain robust even in the presence of corruption is critical in practice. 
In response, we propose $\gmm$ -- a herding~\citep{welling2009herding} style greedy algorithm -- that {\em yields a $k$-subset such that the mean of the subset approximates the geometric median of the (potentially) noisy dataset}. Theoretically, we show that $\gm$ Matching enjoys an improved $\gO(1/k)$ scaling over $\gO(1/\sqrt{k})$ scaling of uniform sampling; while achieving the optimal breakdown point of 1/2 even under arbitrary corruption. Extensive experiments across popular deep learning benchmarks indicate that $\gm$ Matching consistently outperforms prior state-of-the-art; the gains become more profound at high rates of corruption and aggressive pruning rates; making it a strong baseline for robust data pruning.

% OLD BACKUP:
% Data pruning, the combinatorial task of selecting a small and informative subset from a large dataset, is crucial for mitigating the enormous computational costs associated with training data-hungry modern deep learning models at scale. Since, large-scale data collections are invariably noisy; developing data pruning strategies that remain robust even in the presence of corruption is critical in practice. Unfortunately, however the existing heuristics for (robust) data pruning lack theoretical coherence and rely on heroic assumptions, that are, often unattainable, by the very nature of the problem setting. Moreover, these strategies often yield sub-optimal neural scaling law even compared to random sampling, especially in scenarios involving strong corruption and aggressive pruning rates -- making provably robust data pruning an open challenge. In response, in this work, we propose Geometric Median (\gm) Matching -- a herding style algorithm that yields a $k$-subset such that the mean of the subset approximates the geometric median of the noisy dataset. Theoretically, we show that $\gm$ Match enjoys an improved $\gO(1/k)$ scaling over $\gO(1/\sqrt{k})$ scaling of uniform sampling; while achieving {\bf optimal breakdown point} of {\bf 1/2} even under {\bf arbitrary} corruption. Extensive experiments across several popular deep learning benchmarks indicate that $\gm$ Matching consistently improves over prior state-of-the-art; the gains become more profound at high rates of corruption and aggressive pruning rates; making $\gm$ Matching a strong baseline for future research in robust data pruning.
% We perform a battery of experiments of training ResNet-18/50, CLIP-ViTB-16/32, 
% across medium to large scale datasets e.g. CIFAR10/100, Mini-ImageNet, ImageNet-1k under different 

==> ICLR-2025/main-paper/algo.tex <==
\begin{algorithm}
\SetAlgoLined
{\bf Initialize :} A finite collection of $\alpha$ corrupted (\cref{def:corruption_model}) observations $\gD$ defined over Hilbert space $\gH \in \sR^d$, equipped with norm $\|\cdot\|$ and inner $\langle\cdot\rangle$ operators; initial weight vector $\vtheta_0 \in \gH$. 
\\
{\bf Robust Mean Estimation:} $\Mu^\gm =\argmin_{\vz\in \gH}\sum_{\vx_i \in \gD}\|\vz - \vx_i\|$
\\
$\gD_\gS \leftarrow \emptyset$
\\
\For{iterations  t = 0, 1, \dots , k-1}
{
    $\vx_{t+1} := \argmax_{\vx \in \gD} \; \langle\vtheta_t,\vx\rangle$
    \\
    $\vtheta_{t+1} := \vtheta_t + \Mu^\gm_\epsilon - \vx_{t+1}$
    \\
    $\gD_\gS := \gD_\gS \cup \vx_{t+1}$
    \\
    $\gD: = \gD \setminus \vx_{t+1}$
}
{\bf return:} $\gD_\gS$
\caption{\bf\textsc{Geometric Median Matching}}
\label{algo:gmm}
\end{algorithm}

==> ICLR-2025/main-paper/exp.tex <==
In this section, we outline our experimental setup, present our key empirical findings, and discuss deeper insights into the performance of $\gm$ Matching. Due to space constraint we only present a subset of the results in the main paper. Please refer to~\cref{sec:appendix}, for additional experimental evidence.

\input{NeuRips-2024/main-paper-tables/tab-main-clean}

{\bf \textsc{Baselines}:} 
\quad
To ensure reproducibility, our experimental setup is identical to~\citep{xia2022moderate}. We compare the proposed $\gm$ Matching selection strategy against the following popular data pruning strategies as baselines for comparison:  (1) Random; (2) Herding \cite{welling2009herding}; (3) Forgetting \cite{toneva2018empirical}; (4) GraNd-score \cite{paul2021deep}; (5) EL2N-score \cite{paul2021deep}; (6) Optimization-based \cite{yang2022dataset}; (7) Self-sup.-selection \cite{sorscher2022beyond} and (8) Moderate~\citep{xia2022moderate}. We do not run these baselines for be these baselines are borrowed from~\citep{xia2020robust}. Additionally, for further ablations we compare $\gm$ Matching with many (natural) distance based geometric pruning strategies: ({\bf \textsc{Uniform}}) Random Sampling, ({\bf \textsc{Easy}}) Selection of samples closest to the centroid; ({\bf \textsc{Hard}}) Selection of samples farthest from the centroid; ({\bf \textsc{Moderate}})~\citep{xia2022moderate} Selection of samples closest to the median distance from the centroid; ({\bf \textsc{Herding}}) Moment Matching~\citep{chen2010super}, ({\bf \textsc{GM Matching}}) Robust Moment (GM) Matching~\eqref{eq:gm_matching}.

\input{NeuRips-2024/main-paper-tables/tab-main-image-corr}

{\bf \textsc{Datasets and Networks}:}
\quad
We perform extensive experiments across three popular image classification datasets - CIFAR10, CIFAR100 and Tiny-ImageNet. Our experiments span popular deep nets including ResNet-18/50~\citep{he2016deep}, VGG-16~\citep{simonyan2014very}, ShuffleNet~\citep{ma2018shufflenet}, SENet~\citep{hu2018squeeze}, EfficientNet-B0\citep{tan2019efficientnet}. 

{\bf \textsc{Implementation Details}:}
\quad
For the CIFAR-10/100 experiments, we utilize a batch size of 128 and employ SGD optimizer with a momentum of 0.9, weight decay of 5e-4, and an initial learning rate of 0.1. The learning rate is reduced by a factor of 5 after the 60th, 120th, and 160th epochs, with a total of 200 epochs. Data augmentation techniques include random cropping and random horizontal flipping. In the Tiny-ImageNet experiments, a batch size of 256 is used with an SGD optimizer, momentum of 0.9, weight decay of 1e-4, and an initial learning rate of 0.1. The learning rate is decreased by a factor of 10 after the 30th and 60th epochs, with a total of 90 epochs. Random horizontal flips are applied for data augmentation. Each experiment is repeated over 5 random seeds and the variances are noted. Throughout this paper, we use Weiszfield Solver~\citep{weiszfeld1937point} to compute $\gm$ approximately.

{\bf \textsc{Proxy Model}:}
\quad
Needless to say, identifying sample importance is an ill-posed problem without some notion of similarity among the samples. Thus, it is common to assume access to a proxy encoder 
that maps the features to a separable embedding space 
% Hilbert space equiped with inner product. Intuitively, this simply means that the embedding space of the encoder fosters proximity of semantically similar examples, while enforcing the separation of dissimilar ones 
-- a property often satisfied by off-the-shelf pretrained foundation models~\citep{hessel2021clipscore, sorscher2022beyond}. We perform experiments across multiple choices of such proxy encoder scenarios: {\bf (A) Standard Setting: } when the proxy model shares the same architecture as the model~\cref{tab:main-clean}-~\ref{tab:main-A}). Additionally, we also experiment with {\bf (B) Distribution Shift: } proxy model pretrained on a different (distribution shifted) dataset(~\cref{fig:main-cifar-vanilla}-\ref{fig:main-cifar-lp}) e.g. ImageNet and used to sample from CIFAR10. {\bf (C) Network Transfer: } where, the proxy has a different network compared to the downstream classifier (\cref{tab:main-nw-T}).

\textsc{Ideal (No Corruption) Scenario}

Our first sets of experiments involve performing data pruning across selection ratio ranging from 20\% - 80\% in the uncorrupted setting. The corresponding results, presented in~\cref{tab:main-clean}, indicate that while $\gm$ Matching is developed with robustness scenarios in mind, it outperforms the existing strong baselines even in the clean setting. Overall, on both CIFAR-100 and Tiny ImageNet $\gm$ Matching improves over the prior methods > 2\% on an average. In particular, we note that $\gm$ Matching enjoys larger gains in the low data selection regime, while staying competitive at low pruning rates.
\input{NeuRips-2024/main-paper-tables/tab-main-label-corr}

\textsc{Corruption Scenarios}

To understand the performance of data pruning strategies in presence of corruption, we experiment with three different sources of corruption -- image corruption, label noise and adversarial attacks. 

{\bf \textsc{Robustness to Image Corruption}:} 
\quad
In this set of experiments, we investigate the robustness of data pruning strategies when the input images are corrupted -- a popular robustness setting, often encountered when training models on real-world data~\citep{hendrycks2019benchmarking, szegedy2013intriguing}.
To corrupt images, we apply five types of realistic noise: Gaussian noise, random occlusion, resolution reduction, fog, and motion blur to parts of the corrupt samples i.e. to say if $m$ samples are corrupted, each type of noise is added to one a random $m/5$ of them, while the other partitions are corrupted with a different noise. The results are presented in~\cref{tab:main-C}. We observe that $\gm$ Matching outperforms all the baselines across all pruning rates improving $\approx $3\% across both datasets on an average. We note that, the gains are more consistent and profound in this setting over the clean setting. Additionally, similar to our prior observations in the clean setting, the gains of $\gm$ Matching are more significant at high pruning rates.

\input{NeuRips-2024/main-paper-tables/tab-main-A}

{\bf \textsc{Robustness to Label Corruption}:}
\quad
Next, we consider another important corruption scenario where a fraction of the training examples are mislabeled. 
% Since acquiring manually labeled data is often impractical and data in the wild always contains noisy annotations -- it is important to ensure the pruning method is robust to label noise. 
We conduct experiments with synthetically injected symmetric label noise~\citep{li2022selective, patrini2017making, xia2020robust}. The results are summarized in~\cref{tab:main-N}. Encouragingly, $\gm$ Matching {\bf outperforms the baselines by $\approx$ 12\%}. Since, mislabeled samples come from different class - they tend to be spatially quite dissimilar, being less likely to be picked by $\gm$ matching, explaining the superior performance.

\input{NeuRips-2024/main-paper-tables/tab-main-nw-transfer}

{\bf \textsc{Robustness to Adversarial Attacks}:}
\quad
Finally, we experiment with adversarial attacks that add imperceptible but adversarial noise on natural examples~\citep{szegedy2013intriguing, huang2010active}. Specifically, we employ two popular adversarial attack algorithms -- PGD attack~\citep{madry2017towards} and GS Attacks~\citep{goodfellow2014explaining} on models trained with CIFAR-100 and Tiny-ImageNet to generate adversarial examples. Following this, various pruning methods are applied to these adversarial examples, and the models are retrained on the curated subset of data. The results are summarized in~\cref{tab:main-A}. Similar to other corruption scenarios, even in this setting, $\gmm$ outperforms the baselines yielding $\approx$ 3\% average gain over the best performing baseline.

\input{plots/CIFAR-10-Scratch-Label-Noise/main-fig}

\textsc{Generalization to Unseen Network / Domain}

Since, the input features (e.g. images) often reside on a non-separable manifold, data pruning strategies rely on a proxy model to map the samples into a separable manifold (embedding space), wherein the data pruning strategies can now assign importance scores. However, it is important for the data pruning strategies to be robust to architecture changes i.e. to say that samples selected via a proxy network should generalize well when trained on unseen (during sample selection) networks / domains. We perform experiments on two such scenarios: 

\input{plots/CIFAR10-LP-Label-Noise/main-fig}

{\bf \textsc{Network Transfer}:} 
\quad
In this setting, the proxy model is trained on the target dataset (no distribution shift). However, the proxy architecture is different than the downstream network. In~\cref{tab:main-nw-T}, we use a ResNet-50 proxy trained on Mini-ImageNet to sample the data. However, then we train a downstream SENet and EfficientNet-B0 on the sampled data.

{\bf \textsc{Domain Transfer}:} 
\quad
Next, we consider the setting where the proxy shares the same architecture with the downstream model. However, the proxy used to select the samples is pretrained on a different dataset (distribution shift) than target dataset. In~\cref{fig:main-cifar-vanilla} we use a proxy ResNet-18 pretrained on ImageNet to select samples from CIFAR10. The selected samples are used to train a subsequent ResNet-18. In~\cref{fig:main-cifar-lp}, we additionally freeze the pretrained encoder i.e. we use ResNet-18 encoder pretrained on ImageNet as proxy. Further, we freeze the encoder and train a downstream linear classifier on top over CIFAR-10. 








==> ICLR-2025/main-paper/gmm.tex <==
Despite its strong performance guarantees in the vanilla (uncorrupted) setting, we argue that the algorithm can result in arbitrarily poor solution in the noisy setting. The vulnerability can be attributed to the estimation of target moment via empirical mean -- notorious for its sensitivity to outliers. Consider a single adversarial sample: $\vx^\gB = |\gD|\bm{\mu}^\gB - \sum_{\vx \in \gD\setminus\vx^\gB}\vx$, shifting the empirical mean to adversary chosen arbitrary target $\bm{\mu}^\gB$. This implies that the empirical mean can't tolerate even a single grossly corrupted sample i.e. yields {\bf lowest possible asymptotic breakdown point of 0}. As a consequence, optimizing over the moment matching objective~\eqref{eq:moment_matching} no longer guarantees convergence to the true underlying (uncorrupted) moment $\bm{\mu}^\gG = \mathop{\E}_{\vx \in \gD_\gG} \vx$, instead, the algorithm can be hijacked by a single bad sample, warping the solution towards an adversarial target. 

\fcolorbox{black}{white}
{
    \begin{minipage}{0.97\linewidth}
        Motivated by this key observation, a natural idea to enable \textsc{Robust Moment Matching} is to replace the empirical mean in~\eqref{eq:moment_matching} with a robust surrogate estimator of the target moment and perform greedy herding updates to match the robust surrogate. Ideally, the robust estimate $\bm{\mu}$ should ensure that the estimation error $\Delta = \|\bm{\mu} - \bm{\mu}^\gG \| \leq \delta$ remain bounded, even when the observations are $\alpha$-corrupted~(\cref{def:corruption_model}). Moreover, the estimate should reside inside the relative interior of $\gC_\gG = \text{conv}\{\vx | \vx \in \gD_\gG\}$ to ensure the linear convergence guarantee.
    \end{minipage}
}

\input{plots/toy/fig.toy-mean-est-2}

In the univariate setting, various robust mean estimators, such as the median and the trimmed mean, are known to achieve the optimal breakdown point 1/2. A common strategy to extend these methods to the multivariate setting is to perform univariate estimation independently along each dimension. However, in high dimensions, these estimates need not lie in the convex hull of the samples and are not orthogonal equivariant and can even become degenerate in the overparameterized settings ($n \ll d$)~\citep{lopuhaa1991breakdown, rousseeuw2005robust}. On the other hand, \textsc{M}-estimators are affine equivariant but have break-down point at most $1/(d + 1)$~\citep{donoho1983notion}. 

\fcolorbox{black}{white}
{
    \begin{minipage}{0.97\linewidth}
    \begin{definition}[{\textbf{Geometric Median}}]
    \label{def:geo_med}
        Given a finite collection of observations $\{\vx_1, \vx_2, \dots \vx_n\}$ defined over Hilbert space $\gH \in \sR^d$, equipped with norm $\|\cdot\|$ and inner $\langle\cdot\rangle$ operators,
        the geometric median(or Fermat-Weber point)~\citep{weber1929alfred} is defined as:
        \begin{equation}
        \label{eq:gm}
            \bm{\mu}^\gm = \gm(\{\vx_1, \vx_2, \dots \vx_n\}) =\argmin_{\vz\in \gH}\bigg[ \rho(\vz):= \sum_{i=1}^{n}\bigg\|\vz - \vx_i\bigg\|
            \bigg] 
        \end{equation}
    \end{definition}
    \end{minipage}
}

In this context, Geometric Median ($\gm$) (~\cref{def:geo_med}) -- a well studied spatial estimator, known for several nice properties like {\bf rotation and translation invariance} and \textbf{optimal breakdown point of 1/2 under gross corruption}~\citep{minsker2015geometric, kemperman1987median}. Moreover, the estimate is guaranteed to lie in the relative interior of the convex hull of the majority (good) points i.e. $\bm{\mu}^\gm \in \gC_\gG$ making it a natural choice to estimate the target moment.    

Computing the $\gm$ exactly, is known to be hard as linear time algorithm exists~\citep{bajaj1988algebraic}, making it is necessary to rely on approximation methods to estimate the geometric median~\citep{weiszfeld1937point, vardi2000multivariate, cohen2016geometric}. We call a point $\bm{\mu}_\epsilon^\gm \in \gH$ an $\epsilon$ accurate $\gm$ if it holds: 
\begin{equation}
    \sum_{i=1}^{n}\bigg\|\bm{\mu}_\epsilon^\gm - \vx_i\bigg\| \leq (1 + \epsilon)\sum_{i=1}^{n}\bigg\|\bm{\mu}^\gm - \vx_i\bigg\|
\label{eq:gm_epsilon}
\end{equation}
We then, exploit the breakdown and translation invariance property of GM and solve for the following \textsc{Robust Moment Matching} objective -- a robust surrogate of~\eqref{eq:moment_matching}:
\begin{equation}
    \argmin_{\gD_\gS \subseteq \gD, |\gD_\gS| = k}
    \bigg\| \Mu^\gm_\epsilon - \frac{1}{k} \sum_{\vx_i \in \gS}\vx_i\bigg\|^2
\label{eq:gm_matching}
\end{equation}
Consequently, we perform herding style greedy minimization of the error~\eqref{eq:gm_matching} : 

\fcolorbox{black}{white}
{
    \begin{minipage}{0.97\linewidth}
        We start with a suitably chosen $\vtheta_0 \in \sR^d$; and repeatedly perform the following updates, adding one sample at a time, $k$ times:
        \begin{flalign}
            \vx_{t+1} &:= \argmax_{\vx \in \gD} \; \langle\vtheta_t, \vx\rangle
            \label{eq:samle_update_gm}
            \\
            \vtheta_{t+1} &:= \vtheta_t + \bigg( \Mu^\gm_\epsilon - \vx_{t+1} \bigg)
            \label{eq:theta_update_gm}
        \end{flalign}
    \end{minipage}
}

We refer to the resulting robust data pruning approach as $\gmm$. For ease of exposition, let $\vtheta_0 = \Mu^\gm_\epsilon$. Then, at iteration $t=T$, $\gmm$ is performing:
\begin{flalign}
    \vx_{T+1} = \argmax_{\vx \in \gD} \bigg[ \langle \Mu^\gm_\epsilon , \vx \rangle - \frac{1}{T+1} \sum_{t=1}^T \langle \vx, \vx_t \rangle\bigg]
\end{flalign}
Greedy updates in the direction that reduces the accumulated error, encourages the algorithm to explore underrepresented regions of the feature space, {\bf promoting diversity}. By matching the $\gm$ rather than the empirical mean, the algorithm imposes larger penalties on outliers, which lie farther from the core distribution. This encourages $\gmm$ to {\bf prioritize samples near the convex hull of uncorrupted points} $\gC_\gG = \text{conv}\{\phi_\gB(\vx) | \vx \in \gD_\gG\}$. As a result, the algorithm promotes diversity in a balanced manner, effectively exploring different regions of the distribution while avoiding distant, noisy points, thus mitigating the robustness vs. diversity trade-off discussed in \cref{sec:intro}. This makes $\gmm$ an excellent choice for data pruning in the wild.

\textsc{Theoretical Guarantee}

In order to theoretically characterize the convergence behavior of $\gmm$, we first exploit the robustness property of $\gm$ ~\citep{pmlr-v151-acharya22a, cohen2016geometric, chen2017distributed} to get an upper bound on the estimation error w.r.t the underlying true mean. Next, we use the property that $\gm$ is guaranteed to lie in the interior of the convex hull of majority of the samples~\citep{minsker2015geometric, boyd2004convex} which follows from the properties of convex sets. Combining these two results we establish the following convergence guarantee for $\gmm$ :

\fcolorbox{black}{white}
{
    \begin{minipage}{0.97\linewidth}
    \begin{theorem}
        Suppose that, we are given, a set of $\alpha$-corrupted samples $\gD = \gD_\gG \cup \gD_\gB$ (\cref{def:corruption_model}) and an $\epsilon$ approx. $\gm(\cdot)$ oracle~\eqref{eq:gm}. Further assume that $\|\vx\| \leq R \; \forall \vx \in \gD$ for some constant $R$.
        Then, $\gmm$ guarantees that the mean of the selected $k$-subset $\gD_\gS \subseteq \gD$ converges to a $\delta$-neighborhood of the uncorrupted (true) mean $\bm{\mu}^\gG = \E_{\vx \in \gD_\gG}(\vx)$ at the rate $\gO(\frac{1}{k})$ such that:   
        \begin{equation}
        \label{equation:bound-z0-simplified}
            \delta^2 = \E\bigg\|\frac{1}{k} \sum_{\vx_i \in \gD_\gS}\vx_i - \bm{\mu}^\gG\bigg \|^2\leq 
            \frac{8|\gD_\gG|}{(|\gD_\gG|-|\gD_\gB|)^2}\sum_{\vx \in \gD_\gG}\E\bigg\|\vx -\Mu^\gG \bigg\|^2 +\frac{2\epsilon^2}{(|\gD_\gG|-|\gD_\gB|)^2}
        \end{equation}
    \label{th:gm_match_cvg}
    \end{theorem}
\end{minipage}
}

This result suggest that, even in presence of $\alpha$ corruption, the proposed algorithm $\gm$ Matching converges to a neighborhood of the true mean, where the neighborhood radius depends on two terms -- the first term depends on the variance of the uncorrupted samples and the second term depends on how accurately the $\gm$ is calculated. Furthermore the bound holds $\forall \alpha = \gD_\gB / \gD_\gG < 1$ implying $\gm$ Matching remains robust even when half of the samples are arbitrarily corrupted i.e. it achieves the optimal breakdown point of 1/2. The detailed proofs are provided in~\cref{sec:appendix}. 
% \subsubsection*{Proof Outline}
% In order to theoretically characterize the convergence behavior of $\gmm$, we first exploit the robustness property of $\gm$ ~\citep{pmlr-v151-acharya22a, minsker2015geometric, cohen2016geometric, wu2020federated, chen2017distributed} to get an upper bound on the estimation error w.r.t the underlying true mean. 

% We can exploit the robustness property of $\gm$ to get an upper bound on the estimation error incurred by 
% show that the estimation error remains bounded w.r.t the underlying true mean~\citep{pmlr-v151-acharya22a, minsker2015geometric, cohen2016geometric, wu2020federated, chen2017distributed} even even in presence of grossly corrupted samples (unbounded). 
% % Intuitively, if such a subset can be found, the expected cost (e.g. loss / average gradient) over $\gS$ is guaranteed to be close (as characterized in~\cref{th:gm_match_cvg}) to the expected cost over the uncorrupted examples $\gD_\gG$; enabling robust data pruning. 

% This is because, even in presence of grossly corrupted samples (unbounded), $\gm$ remains bounded w.r.t the underlying true mean~\citep{pmlr-v151-acharya22a, minsker2015geometric, cohen2016geometric, wu2020federated, chen2017distributed}.



%  The detailed proofs are provided in~\cref{sec:appendix}.  

% % compute the discrepancy between the empirical distribution of the current samples and the target distribution; and chooses the next sample that most reduces this discrepancy, adding one sample at a time.
% % set of random samples from $\gD$; compute the discrepancy between the empirical distribution of the current samples and the target distribution; and chooses the next sample that most reduces this discrepancy, adding one sample at a time, until the desired number of samples is reached or the discrepancy falls below a certain threshold. Note that, by converting the observed moments into a sequence of pseudo samples, herding diverges from the usual approach of first learning the joint distribution (which is often intractable) and then sampling from that model (which is prone to local mode entrapment). 

% % More formally, suppose we are given a set of samples $\gX = \{\vx_i \in \sR^d \sim p(\rx)\}_{i=1}^N$ from the target distribution; and access to a foundation kernel $\phi_\gB(\cdot)$; then with some suitably chosen weight vector $\vtheta_0 =\phi_\mB(\vx_0 \in \gX) \in \sR^p $ Byzantine Robust Herding repeatedly performs the following updates until convergence:
% % \begin{flalign}
% %     \vx_{t+1} &:= \argmax_{\vx \in \gX} \; \langle\vtheta_t, \phi_\mB(\vx)\rangle\\
% %     \vtheta_{t+1} &:= \vtheta_t + \textsc{Gm}(\phi_\mB(\vx)) - \phi_\mB(\vx_{t+1})
% % \end{flalign}
% % Note that this is simply performing a gradient ascent update along the 

% % Intuitively, this mimics a weakly chaotic non linear dynamical system over the parameter space~\citep{welling2012herding}. 

% % \textcolor{red}{
% % * Use some sort of entropy formulation to characterize diversity. (ISD)
% % \\
% % * Equivalent moment matching objective. (ISD)
% % }

==> ICLR-2025/main-paper/intro.tex <==
Recent success of deep learning has been largely fueled by training gigantic models over vast amounts of training data~\citep{radford2021learning, radford2018improving, brown2020language, kaplan2020scaling, hestness2017deep}. Such large scale training, however is associated with enormous computational costs hindering the path to democratizing AI~\citep{paul2021deep}. Data pruning, the combinatorial task of downsizing a large training set into a small informative subset~\citep{feldman2020core, agarwal2005geometric, muthukrishnan2005data, har2011geometric, feldman2011unified}, is a promising approach for reducing the enormous computational and storage costs of modern deep learning.

\textsc{Existing Data Pruning Strategies}

Consequently, a large body of recent works have been proposed to solve the data selection problem. At a high level, there are two main directions: 
One set of data pruning approaches rely on some carefully designed {\bf pruning metrics}, rank the training samples based on the scores and retain a fraction of them as representative samples (super samples), used for training the downstream model. For example,~\citep{xia2022moderate, joshi2023data, sorscher2022beyond} calculate the importance score of a sample in terms of the distance from the centroid of its corresponding class marginal. Samples closer to the centroid are considered most prototypical (easy) and those far from the centroid are treated as least prototypical (hard). A second set of works reformulate this problem as minimizing a {\bf moment matching} objective~\citep{chen2010super, campbell2018bayesian, dwivedi2021generalized} that aims to select a subset whose mean closely matches that of the entire dataset. 

While this work primarily focuses on spatial approaches, it is worth mentioning that the canonical importance scoring criterion have been proposed in terms gradient norm~\citep{paul2021deep, needell2014stochastic}, uncertainty~\citep{pleiss2020identifying} and forgetfulness~\citep{toneva2018empirical}. Typically, samples closer to the class centroid in feature space tend to have lower gradient norms, exhibit lower uncertainty, and are harder to forget during training. In contrast, samples farther from the centroid generally have higher gradient norms, greater uncertainty, and are easier to forget~\citep{paul2021deep, sorscher2022beyond, xia2022moderate}. Moreover,~\citep{mirzasoleiman2020coresets} extended the moment-matching approach to the gradient space, selecting subsets that preserve the overall gradient statistics of the full dataset.
% \input{plots/toy/fig.toy-trade-off}
% \input{plots/toy/fig.toy-corr=45}

\textsc{Robustness vs Diversity }

\input{plots/toy/fig.toy-corr=40}

In the {\bf ideal scenario} (i.e. in absence of any corruption), hard examples are known to contribute the most in downstream generalization performance~\citep{katharopoulos2018not, joshi2009multi, huang2010active, balcan2007margin} as they often capture most of the usable information in the dataset~\citep{xu2020theory}. On the other hand, in {\bf realistic noisy scenarios} involving outliers, this strategy often fails since the noisy examples are  wrongly deemed informative
for training~\citep{zhang2018generalized, park2024robust}. Pruning methods specifically designed for such noisy scenarios thus propose to retain the most representative (easy) samples~\citep{pleiss2020identifying, jiang2018mentornet, har2006maximum, shah2020choosing, shen2019learning}. However, by only choosing samples far from the decision boundary, these methods ignore the more informative uncorrupted less prototypical samples. This can often result in sub-optimal downstream performance and in fact can also lead to degenerate solutions due to a covariance-shift problem~\citep{sugiyama2012machine}; giving rise to a {\em robustness vs diversity trade off}~\citep{xia2022moderate}. This restricts the applicability of existing pruning methods, as realistic scenarios often deviate from expected conditions, making it challenging or impractical to adjust the criteria and methods accordingly.

\input{ICLR-2025/main-paper/algo}

\textsc{Overview of our approach}

To go beyond these limitations, {\em this paper investigates data pruning in the presence of arbitrary corruption}. Specifically, we consider the $\alpha$ corruption framework (\cref{def:corruption_model}), where $0 \leq \psi < \frac{1}{2}$ fraction of the samples are allowed to be {\bf arbitrarily perturbed}. This allowance for {\bf arbitrary corruption} enables us to generalize many practical robustness scenarios; including \textbf{corrupt feature / label} and {\bf adversarial attacks}. 

We make a key observation that, traditional pruning methods typically use the empirical mean to calculate the centroid of the samples, which then guides the selection process based on how representative those samples are. However, the {\bf empirical mean is highly susceptible to outliers} -- in fact, it is possible to construct a single adversarial example to arbitrarily perturb the empirical mean. As a consequence, in the presence of arbitrary corruption, the conventional distinction between easy (robust) and hard samples breaks down, leading to the selection of subsets that are significantly compromised by corruption as illustrated in \cref{fig:toy-corr=40}, depicting sampling from a corrupted Gaussian. 

In response, we propose a data pruning strategy that fosters balanced diversity, effectively navigating various regions of the distribution while avoiding distant, noisy points. Our key idea is to replace the target moment in the standard moment matching objective with a robust surrogate -- Geometric Median~\citep{weber1929alfred, weiszfeld1937point} -- a classical robust estimator of the mean. In particular, we optimize over finding a subset minimizes the discrepancy between the subset's mean and the $\gm$ (\cref{def:geo_med}) of the (potentially noisy) dataset using greedy herding~\citep{welling2009herding} style update rule. We call our algorithm Geometric Median Matching as described in~\cref{algo:gmm}. 
% Leveraging classical robustness properties of $\gm$, we show that $\gmm$ is guaranteed to linearly converge to a bounded neighborhood of the underlying true (uncorrupted) mean of the dataset even when $1/2$ fraction of the samples are arbitrarily corrupted (~\cref{th:gm_match_cvg}). 

\textsc{Contributions}

Overall, our contributions can be summarized as follows:  
\setlength{\intextsep}{0pt}
\begin{itemize}\setlength \itemsep{0.03 em}
    \item 
    We systematically and formally investigate and extend data pruning in presence of corruption. In particular, we study data pruning under the gross corruption framework (\cref{def:corruption_model}), where up to 1/2 fraction of the training examples are allowed to be arbitrarily corrupted.
    We note that, existing pruning heuristics (including the ones proposed for robust scenarios) break down under this strong corruption, due to empirical mean's vulnerability to corruption (\cref{sec:gm_match}, \cref{fig:toy-corr=40}).

    \item 
    Motivated by this key observation, we exploit the robustness property of $\gm$ (\cref{def:geo_med}), to design a novel robust moment matching objective~\eqref{eq:gm_matching}. It aims at finding a subset such that the mean of the subset approximates the $\gm$ of the noisy dataset. We minimize over this objective using greedy herding~\citep{welling2009herding} style update rule. We call the resulting data pruning algorithm $\gmm$ and formally describe it in~\cref{algo:gmm}.  

    \item Leveraging classical robustness properties of $\gm$, we show that, $\gm$ Matching converges to a bounded neighborhood of original underlying mean, at an impressive $\gO(1/k)$ rate while being robust even when up to 1/2 of the samples are arbitrarily corrupted (~\cref{th:gm_match_cvg}) .

    \item Extensive experiments over CIFAR 10/100, Tiny ImageNet, across feature corruption, label noise and adversarial attacks indicate the superiority of $\gm$ Matching over existing methods. We improve over prior work almost in all settings, the gains are especially more profound (often by more than 10\%) in presence of corruption and at aggressive pruning rates; making GM Matching a strong baseline for future research in robust data pruning.

\end{itemize}



==> ICLR-2025/main-paper/problem_setup.tex <==
Given a set of samples $\gD$, the goal of data pruning is to select a subset of the most representative samples $\gD_\gS \subseteq \gD$, that can approximate the underlying distribution well. Data pruning methods achieve this by first defining a {\em pruning criterion} e.g. based on distance, uncertainty, diversity; and then selecting a subset that best satisfies these criteria to represent the full dataset effectively. If such a subset (also referred to as coreset) can be found in a compute efficient manner, then training a parametric model on the subset, typically yields similar generalization performance as training on the entire dataset while resulting in significant speed up when $|\gD_\gS| \ll |\gD|$. However, for machine learning systems deployed in the wild, $\gD$ is often noisy and imperfect due to the difficulty and expense of obtaining perfect semantic annotations for large amounts of data, adversarial attacks or simply measurement noises. 

%%%%%%%%%%%%%%%%%%%%%%%
\fcolorbox{black}{white}%{LightCyan}
{
    \begin{minipage}{0.97\linewidth}
        \begin{definition}[{\bf $\alpha$-corruption}]
        \label{def:corruption_model}
            Given a set of observations from the original distribution of interest, an adversary is allowed to \textbf{inspect all the samples} and \textbf{arbitrarily perturb} up to $\psi \in [0, \frac{1}{2})$ fraction of them. We refer to a set of samples $\gD = \gD_{\gG} \cup \gD_{\gB}$ as $\alpha$-corrupted , $\alpha:=|\gD_{\gB}|/ |\gD_{\gG}|  = \frac{\psi}{1 - \psi}< 1$ and $\gD_{\gB}$, $\gD_{\gG}$ denote the sets of corrupt and clean samples respectively.
        \end{definition}
    \end{minipage}
}

%%%%%%%%%%%%%%%%%%%%%%%
To this end, this work studies data pruning under the $\alpha$-corruption framework (\cref{def:corruption_model}), where a fraction $\psi \in [0, \frac{1}{2})$ of the samples can be {\bf arbitrarily} corrupted -- a strong corruption model~\citep{diakonikolas2019robust, pmlr-v151-acharya22a} that generalizes the popular {\bf Huber Contamination Model}~\citep{huber1992robust}, as well as the notorious {\bf Byzantine Corruption}~\citep{lamport1982byzantine}. 

\begin{quote}
% \setlength{\leftskip}{0.1cm} % Adjust this length to increase left margin
% \setlength{\rightskip}{0.1cm} % Adjust this length to increase right margin
Given an $\alpha$-corrupted set of observations $\gD = \gD_{\gG} \cup \gD_{\gB}$, the goal of \textsc{Robust Data Pruning} is thus to judiciously select a subset $\gD_\gS \subseteq \gD$
; that {\em encapsulates the the underlying clean (uncorrupted) distribution induced by subset $\gD_{\gG}$ without any a-priori knowledge about the corrupted samples}. 
\end{quote}


We measure the robustness of data pruning algorithms via breakdown point analysis~\citep{donoho1983notion} -- a classic tool in robust optimization to assess the resilience of an estimator. 

\fcolorbox{black}{white}
{
    \begin{minipage}{0.97\linewidth}
    \begin{definition}[{\bf Breakdown Point}]
    \label{def:breakdown_point}
        The breakdown point of an estimator is defined as the smallest fraction of contaminated data that can cause the estimator to result in arbitrarily large errors.
    \end{definition}
\end{minipage}
}

% An estimator with a high breakdown point is considered robust as it can handle a larger amount of contamination before failing. 
In the context of~\cref{def:corruption_model}, we say that an estimator achieves \textbf{ optimal breakdown point 1/2}~\citep{lopuhaa1991breakdown} if it remains robust in presence of $\alpha$-corruption $\forall \; \alpha < 1$. 
% In simple terms, pruning strategies that rely on centroid estimates with a low breakdown point risk selecting a subset $\gD_\gS \subseteq \gD$ that is heavily influenced by corrupted samples, making it a poor representation of the clean data $\gD_\gG$.



==> ICLR-2025/main-paper/theory.tex <==
For ease of exposition, let $\vtheta_0 = \Mu^\gm_\epsilon$. Then, at iteration $t=T$, $\gmm$ is performing:
\begin{flalign}
    \vx_{T+1} = \argmax_{\vx \in \gD} \bigg[ \langle \Mu^\gm_\epsilon , \vx \rangle - \frac{1}{T+1} \sum_{t=1}^T \langle \vx, \vx_t \rangle\bigg]
\end{flalign}
That is, at each iteration, it greedily selects a sample that minimizes the robust moment matching error~\eqref{eq:gm_matching}. 
In order to theoretically characterize the convergence behavior of $\gmm$, we first exploit the robustness property of $\gm$ ~\citep{pmlr-v151-acharya22a, minsker2015geometric, cohen2016geometric, wu2020federated, chen2017distributed} to get an upper bound on the estimation error w.r.t the underlying true mean

We can exploit the robustness property of $\gm$ to get an upper bound on the estimation error incurred by 
show that the estimation error remains bounded w.r.t the underlying true mean~\citep{pmlr-v151-acharya22a, minsker2015geometric, cohen2016geometric, wu2020federated, chen2017distributed} even even in presence of grossly corrupted samples (unbounded). 
% Intuitively, if such a subset can be found, the expected cost (e.g. loss / average gradient) over $\gS$ is guaranteed to be close (as characterized in~\cref{th:gm_match_cvg}) to the expected cost over the uncorrupted examples $\gD_\gG$; enabling robust data pruning. 

This is because, even in presence of grossly corrupted samples (unbounded), $\gm$ remains bounded w.r.t the underlying true mean~\citep{pmlr-v151-acharya22a, minsker2015geometric, cohen2016geometric, wu2020federated, chen2017distributed}.



This result suggest that, even in presence of $\alpha$ corruption, the proposed algorithm $\gm$ Matching converges to a neighborhood of the true mean, where the neighborhood radius depends on two terms -- the first term depend on the variance of the uncorrupted samples and the second term depends on how accurately the $\gm$ is calculated. 

Consequently, we say that $\gm$ Matching achieves the optimal breakdown point 1/2. The detailed proofs are provided in~\cref{sec:appendix}.  

% compute the discrepancy between the empirical distribution of the current samples and the target distribution; and chooses the next sample that most reduces this discrepancy, adding one sample at a time.
% set of random samples from $\gD$; compute the discrepancy between the empirical distribution of the current samples and the target distribution; and chooses the next sample that most reduces this discrepancy, adding one sample at a time, until the desired number of samples is reached or the discrepancy falls below a certain threshold. Note that, by converting the observed moments into a sequence of pseudo samples, herding diverges from the usual approach of first learning the joint distribution (which is often intractable) and then sampling from that model (which is prone to local mode entrapment). 

% More formally, suppose we are given a set of samples $\gX = \{\vx_i \in \sR^d \sim p(\rx)\}_{i=1}^N$ from the target distribution; and access to a foundation kernel $\phi_\gB(\cdot)$; then with some suitably chosen weight vector $\vtheta_0 =\phi_\mB(\vx_0 \in \gX) \in \sR^p $ Byzantine Robust Herding repeatedly performs the following updates until convergence:
% \begin{flalign}
%     \vx_{t+1} &:= \argmax_{\vx \in \gX} \; \langle\vtheta_t, \phi_\mB(\vx)\rangle\\
%     \vtheta_{t+1} &:= \vtheta_t + \textsc{Gm}(\phi_\mB(\vx)) - \phi_\mB(\vx_{t+1})
% \end{flalign}
% Note that this is simply performing a gradient ascent update along the 

% Intuitively, this mimics a weakly chaotic non linear dynamical system over the parameter space~\citep{welling2012herding}. 

% \textcolor{red}{
% * Use some sort of entropy formulation to characterize diversity. (ISD)
% \\
% * Equivalent moment matching objective. (ISD)
% }

==> ICLR-2025/main-paper/warmup.tex <==
In the uncorrupted setting i.e. when $\gD_\gB = \emptyset$, a natural and widely used approach for data pruning is to formulate it as the following combinatorial \textsc{moment matching} objective: 
\begin{equation}
    \argmin_{\gD_\gS \subseteq \gD, |\gD_\gS| = k}
    \bigg\| \frac{1}{|\gD|}\sum_{\vx_i \in \gD}\vx_i - \frac{1}{k} \sum_{\vx_i \in \gD_\gS}\vx_i\bigg\|^2
\label{eq:moment_matching}
\end{equation}
Observe that,~\eqref{eq:moment_matching} is an instance of the famous set function maximization problem -- known to be NP hard via a reduction from $k$-set cover~\citep{feige1998threshold}. Despite its intractability,~\citep{mirzasoleiman2020coresets} 
 demonstrated a transformation into a submodular set cover problem, enabling efficient solution via greedy algorithms~\citep{nemhauser1978analysis, wolsey1982analysis}. The greedy approach: also referred to as kernel herding~\citep{welling2009herding, welling2010statistical} starts with a suitably chosen $\boldsymbol{\theta}_0 \in \sR^d$; and iteratively adds samples via the following update rule:
\begin{flalign}
    \vx_{t+1} &:= \argmax_{\vx \in \gD} \; \langle\vtheta_t, \vx\rangle
    \label{eq:samle_update_mean}
    \\
    \vtheta_{t+1} 
    &:= \vtheta_t + \bigg( \frac{1}{|\gD|}\sum_{\vx_i \in \gD}\vx_i - \vx_{t+1} \bigg)
    \label{eq:theta_update_mean}
\end{flalign}
It's worth noting that this algorithm is an infinite memory, deterministic process as at each iteration T, $\vtheta_T$ encapsulates the entire sampling history: $\vtheta_T = \vtheta_0 + T\bm{\mu} - \sum_{t=1}^T \vx_t$ where $\bm{\mu} = \frac{1}{|\gD|}\sum_{\vx_i \in \gD}\vx_i$. 
Conceptually, $\vtheta_T$ represents the vector pointing towards under-sampled regions of the target distribution induced by $\gD$ at iteration $T$. The algorithm's greedy selection strategy aligns each new sample with $\vtheta$, effectively {\em herding} new points to fill the gaps left by earlier selections. Remarkably,~\citep{chen2010super} showed that this simple greedy update rule achieves an impressive $\gO(1/k)$ convergence rate for~\eqref{eq:moment_matching}, a quadratic improvement over random sampling where the error decreases at the rate $\gO(1/\sqrt{k})$. The result holds if $\|\vx\| \leq R \; \forall \vx \in \gD$ for some constant $R$ and as long as the target moment is in the relative interior of $\gC = \text{conv}\{\vx | \vx \in \gD\}$ (Proposition 1~\citep{chen2010super}).

% \subsubsection*{Vulnerability Under Corruption}
% Despite its strong performance guarantees in the vanilla (uncorrupted) setting, we argue that the algorithm can result in arbitrarily poor solution in the noisy setting. The vulnerability can be attributed to the estimation of target moment via empirical mean -- notorious for its sensitivity to outliers. Consider a single adversarial sample: $\vx^\gB = |\gD|\bm{\mu}^\gB - \sum_{\vx \in \gD\setminus\vx^\gB}\vx$, shifting the empirical mean to adversary chosen arbitrary target $\bm{\mu}^\gB$. This implies that the empirical mean can't tolerate even a single grossly corrupted sample i.e. yields {\bf lowest possible asymptotic breakdown point of 0}. As a consequence, optimizing over the moment matching objective~\eqref{eq:moment_matching} no longer guarantee convergence to the true underlying (uncorrupted) moment, instead the algorithm can be hijacked by a single bad sample, warping the solution toward an adversarial target.   


==> Meta-Report/ack.tex <==
I would like to thank my peer mentors {\bf Bhargav Bhushanam} for his continuous support and helpful discussions; {\bf Ishan Misra} for introducing Data Distillation and related ideas, {\bf Li Jing, Xiaocong Du} and fellow intern {\bf Zirui Liu} for useful feedback on the work.  Additionally, I am grateful to my other mentors at Meta - {\bf Dhruv Choudhary, Arun Kejariwal, Richard Kauffman} and my recruiter {\bf Catie Cohn} for help and support during the internship.

==> Meta-Report/contrastive_coreset.tex <==
\input{figs_meta/algo_diag.tex}
At a high level {\em our approach relies on the fact that self-supervised contrastive losses e.g. infoNCE transforms the data manifold in such a way that semantically similar samples are pulled closer to each other while the dissimilar ones are pushed away from each other}. Our main idea is to leverage this separation property of contrastive representation learning to efficiently select a subset of data. 
\input{figs_meta/coreset_results.tex}

In particular, suppose that we have at our disposal an off-the-shelf encoder $f_p$, referred to as proxy model hereafter, pretrained independently (where $f_p$ is often a smaller or cheaply trained model i.e. for only a few epochs or a model pretrained on ). Then our algorithm proceeds as follows: we obtain embeddings of the unlabeled training samples $X = \{\vx_i\}_{i=1}^n$ using the available proxy model. Intuitively, since the encoder is trained using infoNCE loss would be projecting the data points on a $\ell_2$ hypersphere resulting in better separation between points with different semantic properties than the data manifold. We then cluster the points $f(\vx_i) \; \forall i \in [n]$ using standard k-means clustering and {\em use the cluster centers and distance from the cluster centers to obtain useful core-set of the training data}. We then train the model $f$ using contrastive loss on only this selected coreset. 

Our core-sets have two important components that we describe in detail below:  
\input{figs_meta/kmeans_manifold.tex}
\subsection{Samples mapped near cluster boundary on hypersphere manifold are hard.}
As discussed before, our approach leverages the fact that infoNCE loss~\citep{sohn2016improved, wu2018improving} projects the training samples onto an unit norm hypersphere embedding space - enforcing attractive forces between semantically similar (positive) pairs and repulsive forces between semantically different pairs (negative). Further, note that since the encoded data samples are distributed on the {\em hypersphere manifold}, performing k-means clustering on the hypersphere manifold implies that the samples furthest from the cluster centers are essentially close to the cluster boundaries. Based on this observation, we define a simple metric based on the {\bf distance of a training sample from its nearest cluster center in the embedding space as a measure of hardness of the sample}. 
% After running the k means clustering algorithm on the encoding, we define a simple metric to measure the hardness of each training sample and choose a fraction of the training samples based on this score to form the core-set. 
In particular, for each training sample in the embedding space, we compute the distance from the closest cluster center and use this as our hardness metric where a larger value indicates harder sample. Then we simply keep the desired fraction of samples with {\bf largest} scores. 
A larger value simply means that the point belongs to the boundary of its corresponding cluster implying that the proxy model has high confusion on these samples i.e. these are hard examples. 
\input{figs_meta/cifar_table.tex}
\subsection{Generating super samples.}
Our experiments reveal (see Table ~\ref{tab:cifar10_coreset}) that hard examples result in improved generalization over random coreset selection only when a large coreset is selected. However, when the coreset size is small it is no better than random coreset selection. 

This indicates, while examples on the decision boundary can be useful in learning finer decision boundaries and are probably more important than easy examples, learning the entire model using only the boundary examples is unable to learn important information from the underlying data distribution.

We note that this observation is consistent with prior work ~\citep{kawaguchi2020ordered} on hard example mining in supervised setting, where it is common to follow a curriculum and incorporate hard example only in an iterative fashion i.e. these curriculum learning ideas often train an initial model on the whole data and use hard examples only in subsequent iterations.  

Contrary to this, we ask the question {\em Is it possible to include samples that are representative of the overall data distribution, such that training with the core-set mimic a similar effect as curriculum learning while not needing to do the initial training on all the data to learn a base model}. In our algorithm setting, we hypothesize that the cluster centers (empirical mean of embeddings of all the samples in the cluster) can serve as a good proxy of the overall distribution. 

In particular, we compute the k centers from the k-means clustering results, and at each batch during contrastive training we include these k synthetic samples (since the k centers don't belong to the training set rather a convex combination of samples belonging to the same cluster in the embedding space) in addition to the hard examples obtained from the distance metric.
Our empirical results show that this is able to improve the performance of the model multi-fold over random coreset selection even when we select a very small coreset resulting in more efficient training.

\subsection{Discussion on proxy model.}
% we propose to train $f$ or a smaller proxy model $f_C$ using self supervised loss for small number of iterations. Intuitively, the resulting representation would be projecting the data points on a $\ell_2$ hypersphere resulting in better separation between points with different semantic properties. We then propose to use kernel herding style clustering approach on the $\ell_2$ hypersphere to identify super samples and subsequently use the super samples as our coreset. We then train the original model $f$ using contrastive loss on only this selected coreset. 
\input{figs_meta/corr_proxy.tex}
A major component of our method is the use of a proxy model to identify hard samples and constructing super samples. In traditional active learning and curriculum learning framework, the model being trained is used in an iterative fashion to measure some uncertainty metrics to select core-sets. However when dealing with large scale deep learning models, this can result in expensive coreset selection, dwarfing the computational benefit of training the model on small subset. In supervised setting ~\citep{coleman2019selection} showed that it is possible to instead use a smaller proxy model to compute the pruning score using uncertainty measure.  

In this work, we adopt this idea and use a much lightweight model to serve as proxy for the coreset selection. In particular, we experiment with models trained for different epochs on the whole datasets to serve as proxy. Our ablation studies indicate that models trained for much less epochs might still have high correlation with the larger model, in terms of the pruning score (see Figure ~\ref{figure:proxy_ablation}) and thus possible to use a lightweight proxy model for the coreset selection. 



==> Meta-Report/intro.tex <==
Learning from limited amount of labeled data is a longstanding challenge in modern machine learning research.
Owing to its recent widespread success in both computer vision and natural language processing tasks~\citep{chen2020big, Grill2020BootstrapYO, Radford2021LearningTV, Gao2021SimCSESC, dai2015semi, radford2018improving} 
{\em self-supervised pretraining followed by supervised finetuning} has become the de-facto approach to learn from limited supervision. 
%owing to its widespread success in representation learning for both computer vision and natural language processing tasks.

These approaches typically leverage unlabeled data in a task agnostic manner during pretraining and use the available label information during finetuning~\citep{hinton2006fast, bengio2006greedy, mikolov2013distributed, kiros2015skip, devlin2018bert, Zbontar2021BarlowTS, assran2020supervision}. 


In this context, contrastive training has demonstrated superior performances over supervised methods on various benchmarks. Joint-embedding methods~\citep{chen2020simple, Grill2020BootstrapYO, Zbontar2021BarlowTS, Caron2021EmergingPI} are one the most promising approach for self-supervised representation learning. In contrastive training, the embeddings are trained to be invariant to distortions. To prevent trivial solutions, they apply impulsive force between embeddings from different images. Contrastive loss is shown to be useful in various domains, including natural language processing~\citep{Gao2021SimCSESC}, multi-modal learning~\citep{Radford2021LearningTV}. It has also been shown to benefit supervised learning~\citep{khosla2020supervised}.

\input{figs_meta/lp_ft.tex}

\subsection{Scaling Laws for Self Supervised Learning}
Despite its widespread success across different machine learning tasks, self supervised learning approaches remain resource intensive to train. They often need to be trained on large amount of unlabeled data for several iterations. 

\input{figs_meta/ssl_data_scaling_law.tex}

Such Neural scaling laws~\citep{zhai2022scaling, gordon2021data, hestness2017deep, kaplan2020scaling, henighan2020scaling, hernandez2021scaling} have been explored in many machine learning applications like vision, language, and speech. These empirical studies suggest that generalization performance often falls off as a power law with either the amount of training data, model size, or compute. However, power law scaling is extremely weak and unsustainable.  For example, a drop in error from 3\% to 2\% might require an order of magnitude more data, compute, or energy.  In language modeling with large transformers, a drop in cross entropy loss from about 3.4 to 2.8 requires 10 times more training data (Fig. 1 in ~\citep{kaplan2020scaling}). Also, for large vision transformers, an additional 2 billion pretraining data points (starting from1billion) leads to an accuracy gain on ImageNet of a few percentage points (Fig. 1 in ~\citep{zhai2022scaling}).

To address this issue, in this work we investigate unsupervised core-set selection strategies to accelerate self-supervised training. Formally speaking,  
\emph{
Suppose, we are given unlabeled training dataset $\gX_{tr}\equiv\{\vx_i\}_{i=1}^N \sim p(\rx)$ where $\rx \in \sR^d$, $d \in \sN$is input random variable.  The goal of core-set selection methods is to find a small subset $\gX_s \subset \gX_{tr}$ with $|\gX_{s}| \ll |\gX_{tr}|$ such that a model trained only on the subset approximately matches the generalization performance of the model trained on the entire training dataset, while requiring an order of magnitude less compute resources~\citep{mirzasoleiman2020coresets}.} 
% \emph{Given a large pool of unlabeled samples $\gX$, we want to identify a representative core-set $\gD$ using unsupervised data pruning metrics such that self-supervised training on the core-set results in equally discriminative representation as contrastive training using the entire dataset}. 

While there exist a large body of literature on coreset selection applied to data efficient training; they are mostly limited to supervised~\citep{mirzasoleiman2020coresets} and semi-supervised settings~\citep{killamsetty2021retrieve}. Most of the existing core-set selection based approaches rely on data pruning metrics that require label information limiting their ability to prune data for large-scale foundation models trained on massive unlabeled datasets~\citep{sorscher2022beyond, bommasani2021opportunities}.
% The existing unsupervised data pruning strategies have only been applied to downstream supervised (or semi supervised setting) training and to the best of our knowledge, there is no existing study that explores core-set selection strategies and scaling laws of data pruning for self-supervised training. 
% There are two major challenges: (a)  (b)  

\emph{Thus it remains an open problem to explore {\bf unsupervised} data pruning strategies that can result in significantly small core-sets for downstream self supervised learning}. 


\subsection{Contributions}
Our contributions can be summarized as follows:
\begin{itemize}
    \item We study the scaling laws of contrastive training and show that the pre-training is more sensitive to data scaling than finetuning.
    \item We propose a novel coreset selection approach 
    by leveraging the separation property of contrastive loss on the hypersphere manifold.
    \item For training ResNet-18 on CIFAR 10 dataset our approach maintains the same generalization performance (or even slightly better) while using only 30\% of the gradient compute implying a 3.3X speedup. 
\end{itemize}







==> Meta-Report/related_work.tex <==
\subsection{Self Supervised Representation Learning.}
% Recall that the goal of this paper is to design a contrastive loss that is able to leverage the available supervision in an efficient manner to learn rich representation $g_B(\vx)$ from Positive Unlabeled dataset that is able to discriminate between positive and negative classes.
The main idea of contrastive learning~\citep{sohn2016improved, wu2018improving} is to contrast semantically similar and dissimilar samples -  encouraging the representations of similar pairs to be close and that of the dissimilar pairs to be more orthogonal.   

In particular, at iteration $t$, given a randomly sampled batch $\gD_t = \{\vx_i \sim p(\vx)\}_{i=1}^b$ of b data points, the corresponding {\em multi-viewed batch} consists of 2b data points $\tilde{\gD_t} = \{\vx_i\}_{i=1}^{2b}$ where $\vx_{2i-1}$ and $\vx_{2i}$ are two views of $\vx_i \in \gD_t$ obtained via stochastic augmentations~\citep{tian2020contrastive}. Within the multi-viewed batch, consider an arbitrary augmented data point indexed by $i \in \sI \equiv \{1, \dots, 2b\}$ and let $a(i)$ be the index of the corresponding augmented sample originating from the same source sample. Denote the embedding of sample $\vx_i$ as $\vz_i = g_{B_t}(\vx_i)$, then the {\em self supervised contrastive loss} {\bf infoNCE}~\citep{gutmann2010noise, oord2018representation} is given as:
\begin{equation}
\small 
    \gL_{infoNCE} = \sum_{i \in \sI} \ell_{InfoNCE}^{(i)} = 
    \sum_{i \in \sI} \left[- \log \frac{\exp{(\vz_i} \boldsymbol \cdot \vz_{a(i)}/\tau)}{\sum_{k \in \sI \setminus \{i\}} \exp{(\vz_i\boldsymbol \cdot \vz_k / \tau)}}\right]
\label{eq:nt_xent}
\end{equation}
In this context $\vx_i$ is commonly referred to as the {\em \bf anchor}, $\vx_{a(i)}$ is called {\em \bf positive} and the other $2(b-1)$ samples are considered {\em \bf negatives}.
Simply put, InfoNCE loss pulls the anchor and the positive in the embedding space while pushing away anchor from negatives.

{\bf Projection Layer.} Rather than directly using the output of the encoder $g_B(\vx)$ to contrast samples, it is common practice~\citep{chen2020simple, Zbontar2021BarlowTS, Grill2020BootstrapYO, khosla2020supervised,  assran2020supervision} to feed the representation through a projection network $h_{\theta_{proj}}$ to obtain a lower dimensional representation before comparing the representations i.e. instead of using $\vz_i = g_{B_t}(\vx_i)$, in practice we consider $\vz_i = h_{\theta_{proj}}(g_{B_t}(\vx_i))$. {\em The projector is only used during optimization and discarded during downstream transfer task}.

\subsection{Coreset Selection}
Given a set of points $\sP$ in some metric space, coreset is defined as a representative subset $\sD$ that approximates $\sP$ with respect to some extent measure (e.g. objective function)~\citep{feldman2020core, agarwal2005geometric, muthukrishnan2005data, har2011geometric, feldman2011unified}. More formally, for a set of candidate queries $\sX$ and a measure function {\bf cost}$(\sP, x\in \sX)$, subset $\sD$ is referred to as an $\epsilon$-coreset of $\sP$ if $\forall x \in \sX$, {\bf cost}$(\sD, x)$ is an approximation of {\bf cost}$(\sP, x)$ up to a multiplicative factor of $1 \pm \epsilon$.

Core-set selection methods have found widespread applications across several machine learning problems such as low resource training, active learning, continual learning, neural architecture search and model compression~\citep{ye2020good, liu2019metapruning, agarwal2005geometric, chen2020storage, he2019filter, li2019learning, maalouf2020deep} to name a few.

% In this work we will primarily focus on the using coreset selection approaches to improve the efficiency of training large scale machine learning models. 
% Our problem setting is described as follows: 
% At a high level, these methods aim to identify a representative subset (can be weighted) of the training data such that the subset approximates the joint distribution of the entire training dataset~\citep{welling2009herding, chen2010super}. The initial motivation of finding such subset was to be able to train ML models on the selected subset such that the resulting model generalizes equally well as the model trained on the whole dataset, while requiring an order of magnitude less compute resources~\citep{mirzasoleiman2020coresets}. 

At a high level all the data pruning approaches rely on defining some {\bf pruning metrics} and rank the training samples based on the scores and retain a fraction of them as representative samples (super samples), used for training the downstream model.  

% \paragraph{Supervised Coreset selection}
Most of the data pruning metrics require label information to compute ranking score. Typically they train the model $f$ for a pre-decided number of iterations $T_C$ using the whole dataset to select core-set using the trained model. 
% \paragraph{Geometry Based Methods.}

{\bf A. Geometry Based Methods.} Geometry based approaches rely on the key idea that samples that are close to each other in the feature space tend to have similar semantic properties and often redundant. For example, kernel herding methods~\citep{welling2009herding, chen2010super} select data points based on the distance between the coreset center and original dataset center in the feature space. They incrementally and greedily adds one sample each time into the coreset that can minimize distance between two centers. On the other hand k-center greedy approaches try to solve the mini-max facility location problem~\citep{farahani2009facility}. The problem is NP hard and thus solved using k-center greedy algorithm~\citep{agarwal2020contextual, sener2018active, sinha2020small}.  

{\bf B. Uncertainty based approaches}
These methods argue that samples with lower confidence are harder and may have a
greater impact on model optimization than those with higher confidence and thus should be included in the core-set. Thus, they use the confidence or other metrics that are function of confidence such as entropy, margin to compute pruning score~\citep{coleman2019selection}. 
% We first benchmark different core-set selection selection algorithms on three popular use cases: data efficient ML training, active learning and continual learning. In rest of this section we describe the use cases, tasks and experimental details in more detail.  

{\bf C. Gradient based approaches}
~\citep{mirzasoleiman2020coresets, killamsetty2021grad, killamsetty2021retrieve} try to find a subset of data points via greedy approximation such that the gradient computed on this subset closely follows the gradient of the entire dataset.   

{\bf Selection via proxy}
It is often observed that the accurate coreset selection algorithms itself are expensive thus dwarfing the benefit.~\citep{coleman2019selection} propose to use a smaller model $f_C$ instead of using the original model $f$ for the coresert selection iterations. The intuition is that the solutions are highly correlated to that obtained via $f$.

{\bf Unsupervised Coreset selection}
While, there has been several supervised coreset selection approaches, only a handful of approaches exits that do not require labeled data to compute the pruning score. For example, ~\citep{sorscher2022beyond} try to find cluster centers on the contrastive representation space; ~\citep{ju2022extending} directly uses the correlation between samples computed using infoNCE style loss to find coresets. 

While these methods are closely related to our setting, but note that they unsupervised approaches for coreset selection to improve efficiency of downstream supervised training. Whereas, our setting is to instead explore core-set selection strategies to improve the efficiency of self supervised learning while retaining the quality of produced representations (embeddings).  

Closest to our setting is ~\citep{robinson2020contrastive}, that uses uncertainty based approaches directly on the contrastive loss during contrastive training to identify hard negatives and get rid of easy negatives and show faster convergence - however, note that at each iterations they still need to compute contrastive loss on all the samples in the batch to identify hard negatives implying their per iteration cost is not improved.  






==> NeuRips-2024/abstract.tex <==
Data pruning, the combinatorial task of selecting a small and informative subset from a large dataset, is crucial for mitigating the enormous computational costs associated with training data-hungry modern deep learning models at scale. Since large-scale data collections are invariably noisy, developing data pruning strategies that remain robust even in the presence of corruption is critical in practice. 

Unfortunately, existing heuristics for (robust) data pruning lack theoretical coherence and rely on heroic assumptions, that are, often unattainable, by the very nature of the problem setting. Moreover, these strategies often yield sub-optimal neural scaling laws even compared to random sampling, especially in scenarios involving strong corruption and aggressive pruning rates -- making provably robust data pruning an open challenge. 

In response, in this work, we propose Geometric Median ($\gm$) Matching -- a herding~\citep{welling2009herding} style greedy algorithm -- that {\em yields a $k$-subset such that the mean of the subset approximates the geometric median of the (potentially) noisy dataset}. Theoretically, we show that $\gm$ Matching enjoys an improved $\gO(1/k)$ scaling over $\gO(1/\sqrt{k})$ scaling of uniform sampling; while achieving the optimal breakdown point of 1/2 even under arbitrary corruption. Extensive experiments across popular deep learning benchmarks indicate that $\gm$ Matching consistently outperforms prior state-of-the-art; the gains become more profound at high rates of corruption and aggressive pruning rates; making $\gm$ Matching a strong baseline for future research in robust data pruning.

    % OLD BACKUP:
    % Data pruning, the combinatorial task of selecting a small and informative subset from a large dataset, is crucial for mitigating the enormous computational costs associated with training data-hungry modern deep learning models at scale. Since, large-scale data collections are invariably noisy; developing data pruning strategies that remain robust even in the presence of corruption is critical in practice. Unfortunately, however the existing heuristics for (robust) data pruning lack theoretical coherence and rely on heroic assumptions, that are, often unattainable, by the very nature of the problem setting. Moreover, these strategies often yield sub-optimal neural scaling law even compared to random sampling, especially in scenarios involving strong corruption and aggressive pruning rates -- making provably robust data pruning an open challenge. In response, in this work, we propose Geometric Median (\gm) Matching -- a herding style algorithm that yields a $k$-subset such that the mean of the subset approximates the geometric median of the noisy dataset. Theoretically, we show that $\gm$ Match enjoys an improved $\gO(1/k)$ scaling over $\gO(1/\sqrt{k})$ scaling of uniform sampling; while achieving {\bf optimal breakdown point} of {\bf 1/2} even under {\bf arbitrary} corruption. Extensive experiments across several popular deep learning benchmarks indicate that $\gm$ Matching consistently improves over prior state-of-the-art; the gains become more profound at high rates of corruption and aggressive pruning rates; making $\gm$ Matching a strong baseline for future research in robust data pruning.
    % We perform a battery of experiments of training ResNet-18/50, CLIP-ViTB-16/32, 
    % across medium to large scale datasets e.g. CIFAR10/100, Mini-ImageNet, ImageNet-1k under different 

==> NeuRips-2024/exp.tex <==
In this section, we outline our experimental setup, present our key empirical findings, and discuss deeper insights into the performance of $\gm$ Matching. 

\subsection{Experimental Setup}
{\bf A. Baselines: } 

To ensure reproducibility, our experimental setup is identical to~\citep{xia2022moderate}. We compare the proposed $\gm$ Matching selection strategy against the following popular data pruning strategies as baselines for comparison:  (1) Random; (2) Herding \cite{welling2009herding}; (3) Forgetting \cite{toneva2018empirical}; (4) GraNd-score \cite{paul2021deep}; (5) EL2N-score \cite{paul2021deep}; (6) Optimization-based \cite{yang2022dataset}; (7) Self-sup.-selection \cite{sorscher2022beyond} and (8) Moderate~\citep{xia2022moderate}. We do not run these baselines for be these baselines are borrowed from~\citep{xia2020robust}.

Additionally, for further ablations we compare $\gm$ Matching with many (natural) distance based geometric pruning strategies: ({\bf \textsc{Uniform}}) Random Sampling, ({\bf \textsc{Easy}}) Selection of samples closest to the centroid; ({\bf \textsc{Hard}}) Selection of samples farthest from the centroid; ({\bf \textsc{Moderate}})~\citep{xia2022moderate} Selection of samples closest to the median distance from the centroid; ({\bf \textsc{Herding}}) Moment Matching~\citep{chen2010super}, ({\bf \textsc{GM Matching}}) Robust Moment (GM) Matching~\eqref{eq:gm_matching}.

{\bf B. Datasets and Networks :}

We perform extensive experiments across three popular image classification datasets - CIFAR10, CIFAR100 and Tiny-ImageNet. Our experiments span popular deep nets including ResNet-18/50~\citep{he2016deep}, VGG-16~\citep{simonyan2014very}, ShuffleNet~\citep{ma2018shufflenet}, SENet~\citep{hu2018squeeze}, EfficientNet-B0\citep{tan2019efficientnet}. 

{\bf C. Implementation Details : } 

For the CIFAR-10/100 experiments, we utilize a batch size of 128 and employ SGD optimizer with a momentum of 0.9, weight decay of 5e-4, and an initial learning rate of 0.1. The learning rate is reduced by a factor of 5 after the 60th, 120th, and 160th epochs, with a total of 200 epochs. Data augmentation techniques include random cropping and random horizontal flipping. In the Tiny-ImageNet experiments, a batch size of 256 is used with an SGD optimizer, momentum of 0.9, weight decay of 1e-4, and an initial learning rate of 0.1. The learning rate is decreased by a factor of 10 after the 30th and 60th epochs, with a total of 90 epochs. Random horizontal flips are applied for data augmentation. Each experiment is repeated over 5 random seeds and the variances are noted.

For all the experiments in this paper we use Weiszfield Solver~\citep{weiszfeld1937point} to compute $\gm$ approximately.

{\bf D. Proxy Model :}

Needless to say, identifying sample importance is an ill-posed problem without some notion of similarity among the samples. Thus, it is common to assume access to a proxy encoder $\phi_\mB(\cdot): \sR^d \to \gH \in \sR^p$ that maps the features to a separable Hilbert space equiped with inner product. Intuitively, this simply means that the embedding space of the encoder fosters proximity of semantically similar examples, while enforcing the separation of dissimilar ones -- a property often satisfied by even off-the-shelf pretrained foundation models~\citep{hessel2021clipscore, sorscher2022beyond}. We perform experiments across multiple choices of such proxy encoder scenarios: {\bf A. Standard Setting: } In~\cref{tab:clean}-~\ref{tab:Adv-A}, we show results for the case when the proxy model shares the same architecture as the model e.g. ResNet-50 to be trained downstream, and is pretrained (supervised) on the clean target dataset e.g. TinyImageNet. Additionally, we also experiment with {\bf B. Distribution Shift: } proxy model pretrained on a different (distribution shifted) dataset e.g. ImageNet and used to sample from Mini ImageNet. {\bf C. Network Transfer: } Where, the proxy has a different network compared to the classifier. We describe these setups in more detail in~\cref{sec:proxy_ablations}.

\input{NeuRips-2024/tables/tab-clean}

\subsection{Ideal (No Corruption) Scenario}
Our first sets of experiments involve performing data pruning across selection ratio ranging from 20\% - 80\% in the uncorrupted setting. The corresponding results, presented in~\cref{tab:clean}, indicate that while $\gm$ Matching is developed with robustness scenarios in mind, it outperforms the existing strong baselines even in the clean setting. Overall, on both CIFAR-100 and Tiny ImageNet $\gm$ Matching improves over the prior methods > 2\% on an average. In particular, we note that $\gm$ Matching enjoys larger gains in the low data selection regime, while staying competitive at low pruning rates.

\input{NeuRips-2024/tables/tab-cifarC}
\input{NeuRips-2024/tables/tab-tinyC}

\subsection{Corruption Scenarios}
To understand the performance of data pruning strategies in presence of corruption, we experiment with three different sources of corruption -- image corruption, label noise and adversarial attacks. 

\subsubsection{Robustness to Image Corruption} 
In this set of experiments, we investigate the robustness of data pruning strategies when the input images are corrupted -- a popular robustness setting, often encountered when training models on real-world data~\citep{hendrycks2019benchmarking, szegedy2013intriguing}.
To corrupt images, we apply five types of realistic noise: Gaussian noise, random occlusion, resolution reduction, fog, and motion blur to parts of the corrupt samples i.e. to say if $m$ samples are corrupted, each type of noise is added to one a random $m/5$ of them, while the other partitions are corrupted with a different noise. The results are presented in~\cref{tab:cifarC},~\ref{tab:tinyC}. We observe that $\gm$ Matching outperforms all the baselines across all pruning rates improving $\approx $3\% across both datasets on an average. We note that, the gains are more consistent and profound in this setting over the clean setting. Additionally, similar to our prior observations in the clean setting, the gains of $\gm$ Matching are more significant at high pruning rates (i.e. low selection ratio).

\input{NeuRips-2024/tables/tab-noisy}
\input{NeuRips-2024/tables/tab-noisy-tiny}

\subsubsection{Robustness to Label Corruption}
Next, we consider another important corruption scenario where a fraction of the training examples are mislabeled. Since acquiring manually labeled data is often impractical and data in the wild always contains noisy annotations -- it is important to ensure the pruning method is robust to label noise. We conduct experiments with synthetically injected symmetric label noise~\citep{li2022selective, patrini2017making, xia2020robust}. The results are summarized in~\cref{tab:label-noise},\ref{tab:tinyN}. Encouragingly, $\gm$ Matching {\bf outperforms the baselines by $\approx$ 12\%}. Since, mislabeled samples come from different class - they are spatially quite dissimilar than the correctly labeled ones thus, less likely to be picked by $\gm$ matching, explaining the superior performance.

\input{NeuRips-2024/tables/tab-attacks}
\input{plots/CIFAR-10-Scratch-Label-Noise/main-fig}
\input{plots/CIFAR10-LP-Label-Noise/main-fig}

\subsubsection{Robustness to Adversarial Attacks}

Finally, we investigate the robustness properties of data pruning strategies in presence of adversarial attacks that add imperceptible but adversarial noise on natural examples~\citep{szegedy2013intriguing, ma2018characterizing, huang2010active}. Specifically, we experiment with two popular adversarial attack algorithms -- PGD attack~\citep{madry2017towards} and GS Attacks~\citep{goodfellow2014explaining}. We employ adversarial attacks on models trained with CIFAR-100 and Tiny-ImageNet to generate adversarial examples. Following this, various methods are applied to these adversarial examples, and the models are retrained on the curated subset of data. The results are summarized in~\cref{tab:Adv-A}. Similar to other corruption scenarios, even in this setting, $\gm$ Matching outperforms the baselines $\approx$  and remains effective across different pruning rates yielding $\approx$ 3\% average gain over the best performing baseline.

\input{NeuRips-2024/tables/tab-clean-net-transfer}
\input{NeuRips-2024/tables/tab-vgg-shuffle}

\subsection{Generalization to Unseen Network / Domain}
\label{sec:proxy_ablations}
One crucial component of data pruning is the proxy network. Since, the input features (e.g. images) often reside on a non-separable manifold, data pruning strategies rely on a proxy model to map the samples into a separable manifold (embedding space), wherein the data pruning strategies can now assign importance scores. However, it is important for the data pruning strategies to be robust to architecture changes i.e. to say that samples selected via a proxy network should generalize well when trained on unseen (during sample selection) networks / domains. We perform experiments on two such scenarios: 

{\bf A. Network Transfer:} In this setting, the proxy model is trained on the target dataset (no distribution shift). However, the proxy architecture is different than the downstream network. In~\cref{tab:clean-nw-transfer}, we use a ResNet-50 proxy trained on MiniImageNet to sample the data. However, then we train a downstram SENet and EfficientNet-B0 on the sampled data. In~\cref{tab:VGG-Shuffle}, we use a ResNet-50 pretrained on Mini ImageNet as proxy, whereas we train a VGG-16 and ShuffleNet over the selected samples.

{\bf B. Domain Transfer:} Next, we consider the setting where the proxy shares the same architecture with the downstream model. However, the proxy used to select the samples is pretrained on a different dataset (distribution shift) than target dataset. In~\cref{fig:main-cifar-vanilla} we use a proxy ResNet-18 pretrained on ImageNet to select samples from CIFAT-10. The selected samples are used to train a subsequent ResNet-18. In~\cref{fig:main-cifar-lp}, we additionally freeze the pretrained encoder i.e. we use ResNet-18 encoder pretrained on ImageNet as proxy. Further, we freeze the encoder and train a downstream linear classifier on top over CIFAR-10 (linear probe). 








==> NeuRips-2024/intro.tex <==
Recent success of deep learning has been largely fueled by training gigantic models over vast amounts of training data~\citep{radford2021learning, radford2018improving, brown2020language, kaplan2020scaling, hestness2017deep}. Such large scale training, however is associated with enormous computational costs hindering the path to democratizing AI~\citep{paul2021deep}. 

Data pruning, the combinatorial task of downsizing a large training set into a small informative subset~\citep{feldman2020core, agarwal2005geometric, muthukrishnan2005data, har2011geometric, feldman2011unified}, is a promising approach for reducing the enormous computational and storage costs of modern deep learning.
Consequently, a large body of recent works have been proposed to solve the data selection problem. At a high level, data pruning approaches rely on some carefully designed {\bf pruning metrics} and rank the training samples based on the scores and retain a fraction of them as representative samples (super samples), used for training the downstream model. For example,~\citep{xia2022moderate, joshi2023data, sorscher2022beyond} calculate the importance score of a sample in terms of the distance from the centroid of its corresponding class marginal.
Samples closer to the centroid are considered most prototypical (easy) and those far from the centroid are treated as least prototypical (hard). Canonically, similar scoring criterion have been developed in terms of gradients~\citep{paul2021deep}, uncertainty~\citep{pleiss2020identifying}, forgetfulness~\citep{toneva2018empirical}. It is worth noting that the distance-based score is closely related to the uncertainty / gradient forgetting based score. Samples close (far away) to the class centroid are often associated with smaller (larger) gradient norm ; lower (higher) uncertainty; harder (easier) to forget~\citep{paul2021deep, sorscher2022beyond, xia2022moderate}. 

% \input{plots/toy/fig.toy-trade-off}
% \input{plots/toy/fig.toy-corr=45}

{\bf Robustness vs Diversity :}   In the {\bf ideal scenario} (i.e. in absence of any corruption), hard examples are known to contribute the most in downstream generalization performance~\citep{katharopoulos2018not, joshi2009multi, huang2010active, balcan2007margin} as they often capture most of the usable information in the dataset~\citep{xu2020theory}. On the other hand, in {\bf realistic noisy scenarios} involving outliers, this strategy often fails since the noisy examples are  wrongly deemed informative
for training~\citep{zhang2018generalized, park2024robust}. Pruning methods specifically designed for such noisy scenarios thus propose to retain the most representative (easy) samples~\citep{pleiss2020identifying, jiang2018mentornet, har2006maximum, shah2020choosing, shen2019learning}. However, by only choosing samples far from the decision boundary, these methods ignore the more informative uncorrupted less prototypical samples. This can often result in sub-optimal downstream performance and in fact can also lead to degenerate solutions due to a covariance-shift problem~\citep{sugiyama2012machine}; giving rise to a {\em robustness vs diversity trade off}~\citep{xia2022moderate}.
This issue restricts the applicability of these methods, as realistic scenarios often deviate from expected conditions, making it challenging or impractical to adjust the criteria and methods accordingly.

To go beyond these limitations, 
% orthogonal to existing approaches, we investigate data pruning under the robust optimization lens. In particular, 
in this work, we consider the setting where a fraction of the samples can be {\bf arbitrarily corrupted}(~\cref{def:corruption_model}). We make a {\bf key} observation that in presence of arbitrary corruption, the class center itself can be arbitrarily shifted and in fact need not even lie in the convex hull of the underlying clean samples. That is to say, in the arbitrary corruption scenario, the entire notion of easy (robust) / hard based on heuristic falls apart. We provide a more formal argument in~\cref{sec:brkdwn}. \cref{fig:toy-corr=45} elaborates this over a toy example.  

\input{NeuRips-2024/algo-gmm}

In response, we develop a selection strategy that aims to find subset such that the discrepancy between the mean of subset and the geometric median ($\gm$)(\cref{def:geo_med}) of the (potentially noisy) dataset is minimized. We call this algorithm Geometric Median Matching and describe it in~\cref{sec:gm_match}. We show that $\gm$ Matching is guaranteed to converge to a neighborhood of the underlying true (uncorrupted) mean of the (corrupted) dataset even when $1/2$ fraction of the samples are arbitrarily corrupted. 
% {\em samples close to the center might not be actually robust} and in fact it is 
% the vulnerability of existing pruning strategy can be attributed to the class center estimation, which can often be arbitrarily away from the true  
% This is a very common situation in real world; for example, consider financial problems where we want to predict the value of stock using linear regression. However, the adversary can inject samples (e.g. promotions, online articles with inflated claims about the company), to artificially skew the predicted price. 
% Theoretically optimal approaches operate on the gradient space which is often extremely high dimensional resulting in significant computational bottleneck~\citep{cohen2016geometric, minsker2015geometric}. While, there has been some recent work to improve the efficiency e.g.~\citep{pmlr-v151-acharya22a} performs geometric median over a low-dimensional gradient subspace, computational bottleneck remains an open problem hindering the adaptation of statistically consistent and theoretically robust M estimators for robustifying large scale ML systems.
% In this work, we aim to tackle both the issues of robustness and efficiency simultaneously, as this particularly challenging setting has received little attention~\citep{xia2022moderate}.  

{\bf Contributions}

Overall, our contributions can be summarized as follows:  
\setlength{\intextsep}{0pt}
\begin{itemize}\setlength \itemsep{0.03 em}
    \item 
    We systematically investigate and extend data pruning in presence of corruption. In particular, we study data pruning under the gross corruption framework (~\cref{def:corruption_model}), where up to 1/2 fraction of the training examples are allowed to be arbitrarily corrupted.
    
    
    \item 
    We show that, existing pruning heuristics (including the ones proposed for robust scenarios) break down under this strong corruption.
    In response; exploiting robustness property of Geometric Median; we propose a robust data pruning strategy that we call $\gm$ Matching that remains robust even when up to 1/2 fraction of the samples are arbitrarily corrupted. 

    \item Theoretically, we show that, $\gm$ Matching converges to a neighborhood of original underlying mean, at an impressive $\gO(1/k)$ rate while being robust.

    \item Extensive experiments over CIFAR 10/100, Tiny ImageNet, across feature corruption, label noise and adversarial attacks indicate the superiority of $\gm$ Matching over existing methods. We improve over prior work almost in all settings, the gains are especially more profound in presence of corruption and at aggressive pruning rates. Thus, making GM Matching a strong baseline for future research in robust data pruning.

\end{itemize}



==> NeuRips-2024/main-paper-tables/tab-main-A.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \resizebox{0.8\textwidth}{!}
{
    \begin{tabular}{lccccc}
        \toprule
        & \multicolumn{2}{c}{\bf CIFAR-100 (PGD Attack)} 
        & \multicolumn{2}{c}{\bf CIFAR-100 (GS Attack)} 
        & \\
        \cmidrule(r){2-3} 
        \cmidrule(r){4-5} 
        {\bf Method / Ratio } 
        & 20\% 
        & 30\% 
        & 20\% 
        & 30\% 
        & {\bf Mean $\uparrow$} 
        \\
        \midrule
        Random 
        & 43.23$\pm$0.31 
        & 52.86$\pm$0.34 
        & 44.23$\pm$0.41 
        & 53.44$\pm$0.44 
        & 48.44
        \\
        Herding 
        & 40.21$\pm$0.72 
        & 49.62$\pm$0.65 
        & 39.92$\pm$1.03 
        & 50.14$\pm$0.15 
        & 44.97
        \\
        Forgetting 
        & 35.90$\pm$1.30 
        & 47.37$\pm$0.99 
        & 37.55$\pm$0.53 
        & 46.88$\pm$1.91 
        & 41.93
        \\
        GraNd-score 
        & 40.87$\pm$0.84 
        & 50.13$\pm$0.30 
        & 40.77$\pm$1.11 
        & 49.88$\pm$0.83 
        & 45.41
        \\
        EL2N-score 
        & 26.61$\pm$0.58 
        & 34.50$\pm$1.02 
        & 26.72$\pm$0.66 
        & 35.55$\pm$1.30 
        & 30.85
        \\
        Optimization-based 
        & 38.29$\pm$1.77 
        & 46.25$\pm$1.82 
        & 41.36$\pm$0.92 
        & 49.10$\pm$0.81 
        & 43.75
        \\
        Self-sup.-selection 
        & 40.53$\pm$1.15 
        & 49.95$\pm$0.50 
        & 40.74$\pm$1.66 
        & 51.23$\pm$0.25 
        & 45.61
        \\
        Moderate-DS 
        & 43.60$\pm$0.97 
        & 51.66$\pm$0.39 
        & 44.69$\pm$0.68 
        & 53.71$\pm$0.37 
        & 48.42
        \\
        {\bf $\gm$ Matching}
        & {\bf 45.41 $\pm$0.86}
        & {\bf 51.80 $\pm$1.01}
        & {\bf 49.78 $\pm$0.27}
        & {\bf 55.50 $\pm$0.31}
        & {\bf 50.62}
        \\
        \toprule
        & \multicolumn{2}{c}{\bf Tiny ImageNet (PGD Attack)} 
        & \multicolumn{2}{c}{\bf Tiny ImageNet (GS Attack)} 
        & \\
        \cmidrule(r){2-3} 
        \cmidrule(r){4-5} 
        {\bf Method / Ratio } 
        & 20\% 
        & 30\% 
        & 20\% 
        & 30\% 
        & {\bf Mean $\uparrow$} 
        \\
        \midrule
        Random 
        & 20.93$\pm$0.30 
        & 26.60$\pm$0.98 
        & 22.43$\pm$0.31 
        & 26.89$\pm$0.31 
        & 24.21
        \\
        Herding 
        & 21.61$\pm$0.36 
        & 25.95$\pm$0.19 
        & 23.04$\pm$0.28 
        & 27.39$\pm$0.14 
        & 24.50
        \\
        Forgetting 
        & 20.38$\pm$0.47 
        & 26.12$\pm$0.19 
        & 22.06$\pm$0.31 
        & 27.21$\pm$0.21 
        & 23.94
        \\
        GraNd-score 
        & 20.76$\pm$0.21 
        & 26.34$\pm$0.32 
        & 22.56$\pm$0.30 
        & 27.52$\pm$0.40 
        & 24.30
        \\
        EL2N-score 
        & 16.67$\pm$0.62 
        & 22.36$\pm$0.42 
        & 19.93$\pm$0.57 
        & 24.65$\pm$0.32 
        & 20.93
        \\
        Optimization-based 
        & 19.26$\pm$0.77 
        & 24.55$\pm$0.92 
        & 21.26$\pm$0.24 
        & 25.88$\pm$0.37 
        & 22.74
        \\
        Self-sup.-selection 
        & 19.23$\pm$0.46 
        & 23.92$\pm$0.51 
        & 19.70$\pm$0.20 
        & 24.73$\pm$0.39 
        & 21.90
        \\
        Moderate-DS 
        & 21.81$\pm$0.37 
        & 27.11$\pm$0.20 
        & 23.20$\pm$0.13 
        & 28.89$\pm$0.27 
        & 25.25
        \\
        {\bf $\gm$ Matching}
        & {\bf 25.98 $\pm$1.12}
        & {\bf 30.77 $\pm$0.25}
        & {\bf 29.71 $\pm$0.45}
        & {\bf 32.88 $\pm$0.73}
        & {\bf 29.84}
        \\
        \bottomrule
    \end{tabular}
    }
    \caption{
    \footnotesize
    {\bf Robustness to Adversarial Attacks}. Comparing (Test Accuracy) pruning methods under PGD and GS attacks. ResNet-50 is used both as proxy and for downstream classification.
    }
    \label{tab:main-A}
\end{table*}


==> NeuRips-2024/main-paper-tables/tab-main-clean.tex <==
\begin{table*}[t]
\footnotesize
\centering
\resizebox{\textwidth}{!}
{
    \begin{tabular}{lccccccc}
        \midrule
        %\rowcolor{light-gray}
        \multicolumn{8}{c}{{\bf CIFAR-100}}
        \\
        \midrule
        {\textbf{Method / Ratio}} 
        & \textbf{20\%} 
        & \textbf{30\%} 
        & \textbf{40\%}
        & \textbf{60\%}
        & \textbf{80\%}
        & \textbf{100\%}
        & \textbf{Mean $\uparrow$}
        \\ 
        \midrule
        Random              
        & 50.26$\pm$3.24 
        & 53.61$\pm$2.73 
        & 64.32$\pm$1.77 
        & 71.03$\pm$0.75 
        & 74.12$\pm$0.56 
        & 78.14$\pm$0.55 
        & 62.67
        \\ 
        Herding               
        & 48.39$\pm$1.42 
        & 50.89$\pm$0.97 
        & 62.99$\pm$0.61 
        & 70.61$\pm$0.44 
        & 74.21$\pm$0.49 
        & 78.14$\pm$0.55 
        & 61.42
        \\ 
        Forgetting            
        & 35.57$\pm$1.40 
        & 49.83$\pm$0.91 
        & 59.65$\pm$2.50 
        & \textbf{73.34$\pm$0.39} 
        & \textbf{77.50$\pm$0.53} 
        & 78.14$\pm$0.55 
        & 59.18
        \\ 
        GraNd-score           
        & 42.65$\pm$1.39 
        & 53.14$\pm$1.28 
        & 60.52$\pm$0.79 
        & 69.70$\pm$0.68 
        & 74.67$\pm$0.79 
        & 78.14$\pm$0.55
        & 60.14
        \\ 
        EL2N-score            
        & 27.32$\pm$1.16 
        & 41.98$\pm$0.54 
        & 50.47$\pm$1.20 
        & 69.23$\pm$1.00 
        & 75.96$\pm$0.88 
        & 78.14$\pm$0.55
        & 52.99
        \\ 
        Optimization-based    
        & 42.16$\pm$3.30 
        & 53.19$\pm$2.14 
        & 58.93$\pm$0.98 
        & 68.93$\pm$0.70 
        & 75.62$\pm$0.33 
        & 78.14$\pm$0.55 
        & 59.77
        \\
        Self-sup.-selection   
        & 44.45$\pm$2.51
        & 54.63$\pm$2.10 
        & 62.91$\pm$1.20 
        & 70.70$\pm$0.82 
        & 75.29$\pm$0.45 
        & 78.14$\pm$0.55 
        & 61.60
        \\ 
        Moderate-DS
        & 51.83$\pm$0.52
        & 57.79$\pm$1.61
        & 64.92$\pm$0.93
        & 71.87$\pm$0.91 
        & 75.44$\pm$0.40 
        & 78.14$\pm$0.55 
        & 64.37
        \\ 
        {\bf $\gm$ Matching}  
        & {\bf 55.93$\pm$ 0.48}
        & {\bf 63.08$\pm$ 0.57}
        & {\bf 66.59$\pm$ 1.18} 
        & 70.82$\pm$ 0.59
        & 74.63$\pm$ 0.86
        & 78.14$\pm$ 0.55  
        & {\bf 66.01}
        \\
        \midrule
        %\rowcolor{light-gray}
        \multicolumn{8}{c}{{\bf Tiny ImageNet}}
        \\
        \midrule
        Random              
        & 24.02$\pm$0.41 
        & 29.79$\pm$0.27 
        & 34.41$\pm$0.46 
        & 40.96$\pm$0.47 
        & 45.74$\pm$0.61 
        & 49.36$\pm$0.25 
        & 34.98 
        \\ 
        Herding               
        & 24.09$\pm$0.45 
        & 29.39$\pm$0.53 
        & 34.13$\pm$0.37 
        & 40.86$\pm$0.61 
        & 45.45$\pm$0.33 
        & 49.36$\pm$0.25 
        & 34.78 
        \\ 
        Forgetting            
        & 22.37$\pm$0.71 
        & 28.67$\pm$0.54 
        & 33.64$\pm$0.32 
        & 41.14$\pm$0.43 
        & \textbf{46.77$\pm$0.31} 
        & 49.36$\pm$0.25 
        & 34.52
        \\ 
        GraNd-score           
        & 23.56$\pm$0.52 
        & 29.66$\pm$0.37 
        & 34.33$\pm$0.50 
        & 40.77$\pm$0.42 
        & 45.96$\pm$0.56 
        & 49.36$\pm$0.25 
        & 34.86 
        \\ 
        EL2N-score            
        & 19.74$\pm$0.26 
        & 26.58$\pm$0.40 
        & 31.93$\pm$0.28 
        & 39.12$\pm$0.46 
        & 45.32$\pm$0.27 
        & 49.36$\pm$0.25 
        & 32.54
        \\ 
        Optimization-based    
        & 13.88$\pm$2.17 
        & 23.75$\pm$1.62 
        & 29.77$\pm$0.94 
        & 37.05$\pm$2.81 
        & 43.76$\pm$1.50 
        & 49.36$\pm$0.25 
        & 29.64
        \\
        Self-sup.-selection   
        & 20.89$\pm$0.42 
        & 27.66$\pm$0.50 
        & 32.50$\pm$0.30 
        & 39.64$\pm$0.39 
        & 44.94$\pm$0.34 
        & 49.36$\pm$0.25 
        & 33.13
        \\ 
        Moderate-DS
        & 25.29$\pm$0.38
        & 30.57$\pm$0.20
        & 34.81$\pm$0.51
        & 41.45$\pm$0.44
        & 46.06$\pm$0.33 
        & 49.36$\pm$0.25 
        & 35.64
        \\ 
        {\bf $\gm$ Matching}  
        & {\bf 27.88$\pm$0.19}
        & {\bf 33.15$\pm$0.26}
        & {\bf 36.92$\pm$0.40}
        & {\bf 42.48$\pm$0.12}
        & 46.75$\pm$0.51
        & 49.36$\pm$0.25 
        & {\bf 37.44}
        \\
        \bottomrule
    \end{tabular}
}
    \caption{
    \footnotesize
    {\bf No Corruption :} Comparing (Test Accuracy) pruning algorithms on CIFAR-100 and Tiny-ImageNet in the uncorrupted setting. ResNet-50 is used both as proxy and for downstream classification.}
    \label{tab:main-clean}
\end{table*}

==> NeuRips-2024/main-paper-tables/tab-main-image-corr.tex <==
\begin{table*}[t]
\footnotesize
\centering
\resizebox{\textwidth}{!}
{
    \begin{tabular}{lccccccc}
        \toprule
        % \rowcolor{light-gray}
        % \multicolumn{8}{c}{{\bf CIFAR-100}}
        % \\
        % \midrule
        {\textbf{Method / Selection ratio}} 
        & \textbf{20\%} 
        & \textbf{30\%} 
        & \textbf{40\%}
        & \textbf{60\%}
        & \textbf{80\%}
        & \textbf{100\%}
        & \textbf{Mean $\uparrow$}
        % \\ 
        % \midrule
        % \multicolumn{8}{c}{{\bf No Corruption}}
        % \\
        % \midrule
        % Random              
        % & 50.26$\pm$3.24 
        % & 53.61$\pm$2.73 
        % & 64.32$\pm$1.77 
        % & 71.03$\pm$0.75 
        % & 74.12$\pm$0.56 
        % & 78.14$\pm$0.55 
        % & 62.67
        % \\ 
        % Herding               
        % & 48.39$\pm$1.42 
        % & 50.89$\pm$0.97 
        % & 62.99$\pm$0.61 
        % & 70.61$\pm$0.44 
        % & 74.21$\pm$0.49 
        % & 78.14$\pm$0.55 
        % & 61.42
        % \\ 
        % Forgetting            
        % & 35.57$\pm$1.40 
        % & 49.83$\pm$0.91 
        % & 59.65$\pm$2.50 
        % & \textbf{73.34$\pm$0.39} 
        % & \textbf{77.50$\pm$0.53} 
        % & 78.14$\pm$0.55 
        % & 59.18
        % \\ 
        % GraNd-score           
        % & 42.65$\pm$1.39 
        % & 53.14$\pm$1.28 
        % & 60.52$\pm$0.79 
        % & 69.70$\pm$0.68 
        % & 74.67$\pm$0.79 
        % & 78.14$\pm$0.55
        % & 60.14
        % \\ 
        % EL2N-score            
        % & 27.32$\pm$1.16 
        % & 41.98$\pm$0.54 
        % & 50.47$\pm$1.20 
        % & 69.23$\pm$1.00 
        % & 75.96$\pm$0.88 
        % & 78.14$\pm$0.55
        % & 52.99
        % \\ 
        % Optimization-based    
        % & 42.16$\pm$3.30 
        % & 53.19$\pm$2.14 
        % & 58.93$\pm$0.98 
        % & 68.93$\pm$0.70 
        % & 75.62$\pm$0.33 
        % & 78.14$\pm$0.55 
        % & 59.77
        % \\
        % Self-sup.-selection   
        % & 44.45$\pm$2.51
        % & 54.63$\pm$2.10 
        % & 62.91$\pm$1.20 
        % & 70.70$\pm$0.82 
        % & 75.29$\pm$0.45 
        % & 78.14$\pm$0.55 
        % & 61.60
        % \\ 
        % Moderate-DS
        % & 51.83$\pm$0.52
        % & 57.79$\pm$1.61
        % & 64.92$\pm$0.93
        % & 71.87$\pm$0.91 
        % & 75.44$\pm$0.40 
        % & 78.14$\pm$0.55 
        % & 64.37
        % \\ 
        % {\bf $\gm$ Matching}  
        % & {\bf 55.93$\pm$ 0.48}
        % & {\bf 63.08$\pm$ 0.57}
        % & {\bf 66.59$\pm$ 1.18} 
        % & 70.82$\pm$ 0.59
        % & 74.63$\pm$ 0.86
        % & 78.14$\pm$ 0.55  
        % & {\bf 66.01}
        % \\
        % \midrule
        % \multicolumn{8}{c}{{\bf 5\% Feature Corruption}}
        % \\
        % \midrule
        % Random              
        % & 43.14$\pm$3.04 
        % & 54.19$\pm$2.92 
        % & 64.21$\pm$2.39 
        % & 69.50$\pm$1.06 
        % & 72.90$\pm$0.52 
        % & 77.26$\pm$0.39 
        % & 60.79
        % \\ 
        % Herding               
        % & 42.50$\pm$1.27 
        % & 53.88$\pm$3.07 
        % & 60.54$\pm$0.94 
        % & 69.15$\pm$0.55 
        % & 73.47$\pm$0.89 
        % & 77.26$\pm$0.39 
        % & 59.81
        % \\ 
        % Forgetting            
        % & 32.42$\pm$0.74 
        % & 49.72$\pm$1.64 
        % & 54.84$\pm$2.20 
        % & 70.22$\pm$2.00 
        % & 75.19$\pm$0.40 
        % & 77.26$\pm$0.39 
        % & 56.48
        % \\ 
        % GraNd-score           
        % & 42.24$\pm$0.57 
        % & 53.48$\pm$0.76 
        % & 60.17$\pm$1.66 
        % & 69.16$\pm$0.81 
        % & 73.35$\pm$0.81 
        % & 77.26$\pm$0.39 
        % & 59.68
        % \\ 
        % EL2N-score            
        % & 26.13$\pm$1.75 
        % & 39.01$\pm$1.42 
        % & 49.89$\pm$1.87 
        % & 68.36$\pm$1.41 
        % & 73.10$\pm$0.36 
        % & 77.26$\pm$0.39 
        % & 51.30
        % \\ 
        % Optimization-based    
        % & 38.25$\pm$3.04 
        % & 50.88$\pm$6.07 
        % & 57.26$\pm$0.93 
        % & 68.02$\pm$0.39 
        % & 73.77$\pm$0.56 
        % & 77.26$\pm$0.39 
        % & 57.64
        % \\
        % Self-sup.-selection   
        % & 44.24$\pm$0.48 
        % & 55.99$\pm$1.21 
        % & 61.03$\pm$0.59 
        % & 69.96$\pm$1.07 
        % & 74.56$\pm$1.17 
        % & 77.26$\pm$0.39 
        % & 61.16
        % \\ 
        % Moderate-DS
        % & 46.78$\pm$1.90
        % & 57.36$\pm$1.22 
        % & 65.40$\pm$1.19
        % & 71.46$\pm$0.19 
        % & {\bf 75.64$\pm$0.61} 
        % & 77.26$\pm$0.39
        % & 63.33
        % \\
        % {\bf $\gm$ Matching}
        % & {\bf 49.50$\pm$0.72}
        % & {\bf 60.23$\pm$0.88}
        % & {\bf 66.25$\pm$0.51}
        % & {\bf 72.91$\pm$0.26}
        % & 75.10$\pm$0.29
        % & 77.26$\pm$0.39
        % & {\bf 64.80}
        % \\
        % \midrule
        % \multicolumn{8}{c}{{\bf 10\% Feature Corruption}}
        % \\
        % \midrule
        % Random              
        % & 43.27$\pm$3.01 
        % & 53.94$\pm$2.78 
        % & 62.17$\pm$1.29 
        % & 68.41$\pm$1.21 
        % & 73.50$\pm$0.73 
        % & 76.50$\pm$0.63 
        % & 60.26
        % \\ 
        % Herding               
        % & 44.34$\pm$1.07 
        % & 53.31$\pm$1.49 
        % & 60.13$\pm$0.38 
        % & 68.20$\pm$0.74 
        % & 74.34$\pm$1.07 
        % & 76.50$\pm$0.63 
        % & 60.06
        % \\ 
        % Forgetting            
        % & 30.43$\pm$0.70 
        % & 47.50$\pm$1.43 
        % & 53.16$\pm$0.44 
        % & 70.36$\pm$0.82 
        % & 75.11$\pm$0.71 
        % & 76.50$\pm$0.63 
        % & 55.31
        % \\ 
        % GraNd-score           
        % & 36.36$\pm$1.06 
        % & 52.26$\pm$0.66 
        % & 60.22$\pm$1.39 
        % & 68.96$\pm$0.62 
        % & 72.78$\pm$0.51 
        % & 76.50$\pm$0.63 
        % & 58.12
        % \\ 
        % EL2N-score            
        % & 21.75$\pm$1.56 
        % & 30.80$\pm$2.23 
        % & 41.06$\pm$1.23 
        % & 64.82$\pm$1.48 
        % & 73.47$\pm$1.30 
        % & 76.50$\pm$0.63 
        % & 46.38
        % \\ 
        % Optimization-based    
        % & 37.22$\pm$0.39 
        % & 48.92$\pm$1.38 
        % & 56.88$\pm$1.48 
        % & 67.33$\pm$2.15 
        % & 72.94$\pm$1.90 
        % & 76.50$\pm$0.63 
        % & 56.68
        % \\
        % Self-sup.-selection   
        % & 42.01$\pm$1.31 
        % & 54.47$\pm$1.19 
        % & 61.37$\pm$0.68 
        % & 68.52$\pm$1.24 
        % & 74.73$\pm$0.36 
        % & 76.50$\pm$0.63 
        % & 60.22
        % \\ 
        % Moderate-DS
        % & 47.02$\pm$0.66 
        % & 55.60$\pm$1.67 
        % & 62.18$\pm$1.86
        % & 71.83$\pm$0.78
        % & {\bf 75.66$\pm$0.66}
        % & 76.50$\pm$0.63
        % & 62.46
        % \\
        % {\bf $\gm$ Matching}
        % & {\bf 48.86$\pm$1.02}
        % & {\bf 60.15$\pm$0.43}
        % & {\bf 66.92$\pm$0.28}
        % & {\bf 72.03$\pm$0.38}
        % & 73.71$\pm$0.19
        % & 76.50$\pm$0.63
        % & {\bf 64.33}
        \\
        \midrule
        \multicolumn{8}{c}{{\bf CIFAR-100 with 20\% corrupted images}}
        \\
        \midrule
        Random              
        & 40.99$\pm$1.46 
        & 50.38$\pm$1.39 
        & 57.24$\pm$0.65 
        & 65.21$\pm$1.31 
        & 71.74$\pm$0.28 
        & 74.92$\pm$0.88 
        & 57.11
        \\ 
        Herding               
        & 44.42$\pm$0.46 
        & 53.57$\pm$0.31 
        & 60.72$\pm$1.78 
        & 69.09$\pm$1.73 
        & 73.08$\pm$0.98 
        & 74.92$\pm$0.88 
        & 60.18
        \\ 
        Forgetting            
        & 26.39$\pm$0.17 
        & 40.78$\pm$2.02 
        & 49.95$\pm$2.31 
        & 65.71$\pm$1.12 
        & 73.67$\pm$1.12 
        & 74.92$\pm$0.88 
        & 51.30
        \\ 
        GraNd-score           
        & 36.33$\pm$2.66 
        & 46.21$\pm$1.48 
        & 55.51$\pm$0.76 
        & 64.59$\pm$2.40 
        & 70.14$\pm$1.36 
        & 74.92$\pm$0.88 
        & 54.56
        \\ 
        EL2N-score            
        & 21.64$\pm$2.03 
        & 23.78$\pm$1.66 
        & 35.71$\pm$1.17 
        & 56.32$\pm$0.86 
        & 69.66$\pm$0.43 
        & 74.92$\pm$0.88 
        & 41.42
        \\ 
        Optimization-based    
        & 33.42$\pm$1.60 
        & 45.37$\pm$2.81 
        & 54.06$\pm$1.74 
        & 65.19$\pm$1.27 
        & 70.06$\pm$0.83 
        & 74.92$\pm$0.88 
        & 54.42
        \\
        Self-sup.-selection   
        & 42.61$\pm$2.44 
        & 54.04$\pm$1.90 
        & 59.51$\pm$1.22 
        & 68.97$\pm$0.96 
        & 72.33$\pm$0.20 
        & 74.92$\pm$0.88 
        & 60.01
        \\ 
        Moderate-DS
        & 42.98$\pm$0.87
        & 55.80$\pm$0.95
        & 61.84$\pm$1.96
        & 70.05$\pm$1.29 
        & 73.67$\pm$0.30
        & 74.92$\pm$0.88
        & 60.87
        \\
        {\bf $\gm$ Matching}
        & {\bf 47.12$\pm$0.64}
        & {\bf 59.17$\pm$0.92}
        & {\bf 63.45$\pm$0.34}
        & {\bf 71.70$\pm$0.60}
        & {\bf 74.60$\pm$1.03}
        & 74.92$\pm$0.88
        & {\bf 63.21}
        \\
        \midrule
        \multicolumn{8}{c}{{\bf Tiny ImageNet with 20 \% corrupted images}}
        \\
        \midrule
        Random              
        & 19.99$\pm$0.42 
        & 25.93$\pm$0.53 
        & 30.83$\pm$0.44 
        & 37.98$\pm$0.31 
        & 42.96$\pm$0.62 
        & 46.68$\pm$0.43 
        & 31.54
        \\ 
        Herding               
        & 19.46$\pm$0.14 
        & 24.47$\pm$0.33 
        & 29.72$\pm$0.39 
        & 37.50$\pm$0.59 
        & 42.28$\pm$0.30 
        & 46.68$\pm$0.43 
        & 30.86
        \\ 
        Forgetting            
        & 18.47$\pm$0.46 
        & 25.53$\pm$0.23 
        & 31.17$\pm$0.24 
        & 39.35$\pm$0.44 
        & 44.55$\pm$0.67 
        & 46.68$\pm$0.43 
        & 31.81
        \\ 
        GraNd-score           
        & 20.07$\pm$0.49 
        & 26.68$\pm$0.40 
        & 31.25$\pm$0.40 
        & 38.21$\pm$0.49 
        & 42.84$\pm$0.72 
        & 46.68$\pm$0.43 
        & 30.53
        \\ 
        EL2N-score            
        & 18.57$\pm$0.30 
        & 24.42$\pm$0.44 
        & 30.04$\pm$0.15 
        & 37.62$\pm$0.44 
        & 42.43$\pm$0.61 
        & 46.68$\pm$0.43 
        & 30.53
        \\ 
        Optimization-based    
        & 13.71$\pm$0.26 
        & 23.33$\pm$1.84 
        & 29.15$\pm$2.84 
        & 36.12$\pm$1.86 
        & 42.94$\pm$0.52 
        & 46.88$\pm$0.43 
        & 29.06
        \\
        Self-sup.-selection   
        & 20.22$\pm$0.23 
        & 26.90$\pm$0.50 
        & 31.93$\pm$0.49 
        & 39.74$\pm$0.52 
        & 44.27$\pm$0.10 
        & 46.68$\pm$0.43 
        & 32.61
        \\ 
        Moderate-DS
        & 23.27$\pm$0.33 
        & 29.06$\pm$0.36 
        & 33.48$\pm$0.11 
        & 40.07$\pm$0.36 
        & 44.73$\pm$0.39 
        & 46.68$\pm$0.43 
        & 34.12
        \\
        {\bf $\gm$ Matching}
        & {\bf 27.19$\pm$0.92}
        & {\bf 31.70$\pm$0.78}
        & {\bf 35.14$\pm$0.19}
        & {\bf 42.04$\pm$0.31}
        & {\bf 45.12$\pm$0.28} 
        & 46.68$\pm$0.43 
        & {\bf 36.24}
        \\
        \bottomrule
    \end{tabular}
}
    \caption{
    \footnotesize
    {\bf Image Corruption : } Experiments comparing pruning methods when 20\% of the images are corrupted. ResNet-50 is used for both proxy (data pruning) and downstream training.
    }
    \label{tab:main-C}
\end{table*}


==> NeuRips-2024/main-paper-tables/tab-main-label-corr.tex <==
\begin{table*}
    \footnotesize
    \centering
    \resizebox{0.8\textwidth}{!}
{
    \begin{tabular}{lccccc}
        \toprule
        
        & \multicolumn{2}{c}{\bf CIFAR-100 (Label noise)} 
        & \multicolumn{2}{c}{\bf Tiny ImageNet (Label noise)} 
        & 
        \\
        \cmidrule(r){2-3} 
        \cmidrule(r){4-5} 
        {\bf Method / Ratio }
        & {\bf 20\%} 
        & {\bf 30\%} 
        & {\bf 20\%} 
        & {\bf 30\%} 
        & {\bf Mean $\uparrow$}
        \\
        \midrule
        \multicolumn{6}{c}{\bf 20\% Label Noise}
        \\
        \midrule
        Random 
        & 34.47$\pm$0.64 
        & 43.26$\pm$1.21 
        & 17.78$\pm$0.44 
        & 23.88$\pm$0.42 
        & 29.85
        \\
        Herding 
        & 42.29$\pm$1.75 
        & 50.52$\pm$3.38
        & 18.98$\pm$0.44 
        & 24.23$\pm$0.29 
        &  34.01
        \\
        Forgetting 
        & 36.53$\pm$1.11 
        & 45.78$\pm$1.04 
        & 13.20$\pm$0.38 
        & 21.79$\pm$0.43 
        & 29.33
        \\
        GraNd-score 
        & 31.72$\pm$0.67 
        & 42.80$\pm$0.30 
        & 18.28$\pm$0.32 
        & 23.72$\pm$0.18 
        & 28.05
        \\
        EL2N-score 
        & 29.82$\pm$1.19 
        & 33.62$\pm$2.35 
        & 13.93$\pm$0.69 
        & 18.57$\pm$0.31 
        & 23.99
        \\
        Optimization-based 
        & 32.79$\pm$0.62 
        & 41.80$\pm$1.14
        & 14.77$\pm$0.95 
        & 22.52$\pm$0.77 
        & 27.57
        \\
        Self-sup.-selection 
        & 31.08$\pm$0.78 
        & 41.87$\pm$0.63 
        & 15.10$\pm$0.73 
        & 21.01$\pm$0.36 
        & 27.27
        \\
        Moderate-DS 
        & 40.25$\pm$0.12 
        & 48.53$\pm$1.60 
        & 19.64$\pm$0.40 
        & 24.96$\pm$0.30
        & 31.33
        \\
        {\bf $\gm$ Matching}
        & {\bf 52.64$\pm$0.72}
        & {\bf 61.01$\pm$0.47}
        & {\bf 25.80$\pm$0.37} 
        & {\bf 31.71$\pm$0.24}
        & {\bf 42.79}
        \\
        \midrule
        \multicolumn{6}{c}{\bf 35\% Label Noise}
        \\
        \midrule
        Random 
        & 24.51$\pm$1.34 
        & 32.26$\pm$0.81 
        & 14.64$\pm$0.29 
        & 19.41$\pm$0.45 
        & 22.71
        \\
        Herding 
        & 29.42$\pm$1.54 
        & 37.50$\pm$2.12 
        & 15.14$\pm$0.45 
        & 20.19$\pm$0.45 
        & 25.56
        \\
        Forgetting 
        & 29.48$\pm$1.98 
        & 38.01$\pm$2.21 
        & 11.25$\pm$0.90 
        & 17.07$\pm$0.66 
        & 23.14
        \\
        GraNd-score 
        & 23.03$\pm$1.05 
        & 34.83$\pm$2.01 
        & 13.68$\pm$0.46 
        & 19.51$\pm$0.45 
        & 22.76
        \\
        EL2N-score 
        & 21.95$\pm$1.08 
        & 31.63$\pm$2.84 
        & 10.11$\pm$0.25 
        & 13.69$\pm$0.32 
        & 19.39
        \\
        Optimization-based 
        & 26.77$\pm$0.15 
        & 35.63$\pm$0.92 
        & 12.37$\pm$0.68 
        & 18.52$\pm$0.90 
        & 23.32
        \\
        Self-sup.-selection 
        & 23.12$\pm$1.47 
        & 34.85$\pm$0.68 
        & 11.23$\pm$0.32 
        & 17.76$\pm$0.69 
        & 22.64
        \\
        Moderate-DS 
        & 28.45$\pm$0.53 
        & 36.55$\pm$1.26 
        & 15.27$\pm$0.31 
        & 20.33$\pm$0.28 
        & 25.15
        \\
        {\bf $\gm$ Matching}
        & {\bf 43.33$\pm$ 1.02}
        & {\bf 58.41$\pm$ 0.68}
        & {\bf 23.14$\pm$ 0.92} 
        & {\bf 27.76$\pm$ 0.40}
        & {\bf 38.16}
        \\
        \bottomrule
    \end{tabular}
}
    \caption{
    \footnotesize
    {\bf Robustness to Label Noise:} Comparing (Test Accuracy) pruning methods on CIFAR-100 and TinyImageNet datasets, under 20\% and 35\% Symmetric Label Corruption, at 20\% and 30\% selection ratio. ResNet-50 is used both as proxy and for downstream classification.
    }
    \label{tab:main-N}
\end{table*}

==> NeuRips-2024/main-paper-tables/tab-main-nw-transfer.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \resizebox{0.8\textwidth}{!}
{
    \begin{tabular}{lccccc}
        \toprule
        
        & \multicolumn{2}{c}{\bf ResNet-50→SENet}
        & \multicolumn{2}{c}{\bf ResNet-50→EfficientNet-B0} 
        & \\
        \cmidrule(r){2-3} 
        \cmidrule(r){4-5} 
        {\bf Method / Ratio } 
        & {\bf 20\%} 
        & {\bf 30\%} 
        & {\bf 20\%} 
        & {\bf 30\%} 
        & {\bf Mean $\uparrow$} 
        \\
        \midrule
        Random 
        & 34.13$\pm$0.71 
        & 39.57$\pm$0.53 
        & 32.88$\pm$1.52 
        & 39.11$\pm$0.94 
        & 36.42 
        \\ 
        Herding 
        & 34.86$\pm$0.55 
        & 38.60$\pm$0.68 
        & 32.21$\pm$1.54 
        & 37.53$\pm$0.22 
        & 35.80
        \\
        Forgetting 
        & 33.40$\pm$0.64 
        & 39.79$\pm$0.78 
        & 31.12$\pm$0.21 
        & 38.38$\pm$0.65 
        &  35.67
        \\
        GraNd-score 
        & 35.12$\pm$0.54 
        & 41.14$\pm$0.42 
        & 33.20$\pm$0.67 
        & 40.02$\pm$0.35
        & 37.37
        \\
        EL2N-score 
        & 31.08$\pm$1.11 
        & 38.26$\pm$0.45 
        & 31.34$\pm$0.49 
        & 36.88$\pm$0.32 
        & 34.39
        \\
        Optimization-based 
        & 33.18$\pm$0.52 
        & 39.42$\pm$0.77 
        & 32.16$\pm$0.90 
        & 38.52$\pm$0.50 
        & 35.82
        \\
        Self-sup.-selection 
        & 31.74$\pm$0.71 
        & 38.45$\pm$0.39 
        & 30.99$\pm$1.03 
        & 37.96$\pm$0.77 
        & 34.79
        \\
        Moderate-DS 
        & 36.04$\pm$0.15
        & 41.40$\pm$0.20 
        & 34.26$\pm$0.48 
        & 39.57$\pm$0.29 
        & 37.82
        \\
        {\bf $\gm$ Matching} 
        & {\bf 37.93$\pm$0.23} 
        & {\bf 42.59$\pm$0.29}
        & {\bf 36.31$\pm$0.67}
        & {\bf 41.03$\pm$0.41} 
        & {\bf 39.47}
        \\
        \bottomrule
    \end{tabular}
}
    
    \caption{
    \footnotesize
    {\bf Network Transfer (Clean)} : Tiny-ImageNet Model Transfer Results. A ResNet-50 proxy is used to find important samples which are then used to train SENet and EfficientNet.
    }
    \label{tab:main-nw-T}
\end{table*}


==> NeuRips-2024/method.tex <==
Under the gross contamination framework~(\cref{def:corruption_model}), the vulnerability of pruning algorithms can be attributed to the centroid estimation. Motivated by this {\bf key observation} in this paper we propose $\gmm$ -- a data pruning strategy that remains provably effective even when up to $1/2$ fraction of the samples are arbitrary corrupted without any distributional assumption on the data. 

\fcolorbox{black}{white}
{
    \begin{minipage}{0.95\linewidth}
    $\gmm$ involves two key steps:
    \begin{itemize}
        \item Find an estimate of the centroid $\bm{\mu}$ of training observations such that $\Delta = \|\bm{\mu} - \bm{\mu}^\gG \|$ remains bounded even when the observations are $\alpha$-corrupted~(\cref{def:corruption_model}).
        \item Find a subset $\gS \subseteq \gD$ such that the empirical mean of the subset $\approx \bm{\mu}$.
    \end{itemize}
    \end{minipage}
}

In the rest of this section, we discuss these two key ideas in detail.

\subsection{\textsc{Robust Centroid Estimation}} 
In the univariate setting, various robust mean estimators, such as the median and the trimmed mean, are known to achieve the optimal breakdown point 1/2. To extend these estimators to the multivariate setting, a common approach can be applying the univariate estimators to each dimension independently. However, in high dimensions this can become problematic e.g. when $d > 2$ these estimates need not lie in the convex hull of the samples and are not orthogonal equivariant i.e. do not commute with co-ordinate transform and can become degenerate in overparameterized settings ($n \ll d$)~\citep{lopuhaa1991breakdown, rousseeuw2005robust}. On the other hand, \textsc{M}-estimators are affine equivariant but have breakdown point at most $1/(d + 1)$~\citep{donoho1983notion}. 

\input{plots/toy/fig.toy_mean-estimation}

In this context, Geometric Median ($\gm$) (~\cref{def:geo_med}) is a well studied spatial estimator, known for several nice properties like {\bf rotation and translation invariance} and \textbf{optimal breakdown point of 1/2 under gross corruption}~\citep{minsker2015geometric, kemperman1987median}.

\fcolorbox{black}{white}
{
    \begin{minipage}{0.95\linewidth}
    \begin{definition}[{\textbf{Geometric Median}}]
    \label{def:geo_med}
        Given a finite collection of observations $\{\vx_1, \vx_2, \dots \vx_n\}$ defined over Hilbert space $\gH \in \sR^d$, equipped with norm $\|\cdot\|$ and inner $\langle\cdot\rangle$ operators,
        the geometric median(or Fermat-Weber point)~\citep{weber1929alfred} is defined as:
        \begin{equation}
        \label{eq:gm}
            \vx_* = \textsc{Gm}(\{\vx_1, \vx_2, \dots \vx_n\}) =\argmin_{\vz\in \gH}\bigg[ \rho(\vz):= \sum_{i=1}^{n}\bigg\|\vz - \vx_i\bigg\|
            \bigg] 
        \end{equation}
    \end{definition}

    Computing the $\gm$ exactly is known to be hard and no linear time algorithm exists~\citep{bajaj1988algebraic}. Consequently, it is necessary to rely on approximation methods to estimate the geometric median~\citep{weiszfeld1937point, vardi2000multivariate, cohen2016geometric}. We call a point $\vx_\epsilon \in \gH$ an {\bf $\epsilon$-accurate geometric median} if it holds that: $\rho(\vx_\epsilon) \leq (1 + \epsilon) \rho(\vx_\ast)$ i.e.

    \begin{equation}
        \sum_{i=1}^{n}\bigg\|\vx_\epsilon - \vx_i\bigg\| \leq (1 + \epsilon)\sum_{i=1}^{n}\bigg\|\vx_\ast - \vx_i\bigg\|
    \label{eq:gm_epsilon}
    \end{equation}

    \end{minipage}
}

% For all the experiments in this paper we use Weiszfield Solver~\citep{weiszfeld1937point} to compute $\gm$. We refer the reader to~\cref{sec:app-gm} for more discussion on $\gm$. 
% % Leveraging these key robustness 

% \begin{lemma}
%     Given a set of $\alpha$-corrupted samples $\gD = \gD_\gG \cup \gD_\gB$ (~\cref{def:corruption_model}), pretrained (proxy) encoder $\phi_\mB(\cdot)$ and an $\epsilon$-approx. $\gm(\cdot)$ oracle~\eqref{eq:gm}, then we have: 
%     \begin{equation}
%         \E\bigg\| \bm{\mu}^\gm - \bm{\mu}^\gG\bigg \|^2\leq 
%         \frac{8|\gD_\gG|}{(|\gD_\gG|-|\gD_\gB|)^2}\sum_{\vx \in \gD_\gG}\E\bigg\|\phi_\mB(\vx) -\bm{\mu}^\gG \bigg\|^2 +\frac{2\epsilon^2}{(|\gD_\gG|-|\gD_\gB|)^2}
%         \label{eq:gm_mean_bound}
%      \end{equation}
%      where, $\bm{\mu}^\gm = \gm(\{\phi_\mB(\vx_i | \vx_i \in \gD)\})$ is the $\epsilon$-approximate $\gm$ over the entire ($\alpha$-corrupted) dataset; and $\bm{\mu}^\gG = \frac{1}{|\gD_\gG|}\sum_{\vx_i \in \gD_\gG}\phi_\mB(\vx_i)$ denotes the mean of the (underlying) uncorrupted set. 
%      \label{lemma:gm_mean_bound}
% \end{lemma}

\subsection{\textsc{Sampling via Robust Moment Matching}}
We exploit the breakdown and translation invariance property of $\gm$ to perform subset selection while being resilient to arbitrary corruption. In particular,

\fcolorbox{black}{white}
{
    \begin{minipage}{0.95\linewidth}
        Given a random batch of samples $\gD$ from an $\alpha$ corrupted dataset (~\cref{def:corruption_model}), access to an $\epsilon$ accurate $\gm(\cdot)$ oracle; we aim to find a $k$-subset of samples such that the mean of the selected subset approximately matches the geometric median of the training dataset, i.e. we aim solve:
        \begin{equation}
            \argmin_{\gD_\gS \subseteq \gD, |\gD_\gS| = k}
            \bigg\| \Mu^\gm_\epsilon - \frac{1}{k} \sum_{\vx_i \in \gS}\vx_i\bigg\|^2
            \label{eq:gm_matching}
        \end{equation}
        where, $\Mu^\gm_\epsilon$ denotes the $\epsilon$-approximate $\gm$~\eqref{eq:gm_epsilon} of training dataset $\gD$.
    \end{minipage}
}

Intuitively, if such a subset can be found, the expected cost (e.g. loss / average gradient) over $\gS$ is guaranteed to be close (as characterized in~\cref{th:gm_match_cvg}) to the expected cost over the uncorrupted examples $\gD_\gG$; enabling robust data pruning. This is because, even in presence of grossly corrupted samples (unbounded), $\gm$ remains bounded w.r.t the underlying true mean~\citep{pmlr-v151-acharya22a, minsker2015geometric, cohen2016geometric, wu2020federated, chen2017distributed}.

Note that the proposed {\bf robust moment matching objective}~\eqref{eq:gm_matching} is an instance of the famous set function maximization problem -- known to be NP hard via a reduction from $k$-set cover~\citep{feige1998threshold, nemhauser1978analysis}. In this work, we adopt the iterative, herding~\citep{welling2009herding, chen2010super} style greedy approach to approximately solve~\eqref{eq:gm_matching}. The idea is simple -- 

\fcolorbox{black}{white}
{
    \begin{minipage}{0.95\linewidth}
        We start with a suitably chosen $\vtheta_0 \in \sR^d$; and repeatedly perform the following updates, adding one sample at a time, $k$ times:
        \begin{flalign}
            \vx_{t+1} &:= \argmax_{\vx \in \gD} \; \langle\vtheta_t, \vx\rangle
            \label{eq:samle_update}
            \\
            \vtheta_{t+1} &:= \vtheta_t + \bigg( \Mu^\gm_\epsilon - \vx_{t+1} \bigg)
            \label{eq:theta_update}
        \end{flalign}
    \end{minipage}
}

% At each iteration, $\gmm$ accumulates the discrepancies between the $\gm$ of dataset and empirical mean of the chosen samples; after $T$ iterations: 
% \begin{flalign}
%     \vtheta_{T+1} = \vtheta_0 + \bigg(T \Mu_\epsilon^\gm - \sum_{t=1}^T\vx_t \bigg)
%     \label{eq:theta}
% \end{flalign}
For ease of exposition, let $\vtheta_0 = \Mu^\gm_\epsilon$. Then, at iteration $t=T$, $\gmm$ is performing:
\begin{flalign}
    \vx_{T+1} = \argmax_{\vx \in \gD} \bigg[ \langle \Mu^\gm_\epsilon , \vx \rangle - \frac{1}{T+1} \sum_{t=1}^T \langle \vx, \vx_t \rangle\bigg]
\end{flalign}
Thus, evidently, $\gmm$ is performing greedy minimization of the error~\eqref{eq:gm_matching}. 

Intuitively, at each iteration, $\gmm$ accumulates the discrepancies between the $\gm$ of dataset and empirical mean of the chosen samples. By pointing towards the direction that reduces the accumulated error, $\mathbf{\theta}_t$ guides the algorithm to explore underrepresented regions of the feature space, thus {\bf promoting diversity}. Moreover, by matching {\bf $\gm$ (robust moment)}, the algorithm ensures that far-away points (outliers) suffer larger penalty -- consequently, encouraging $\gmm$ to choose more samples near the convex hull of uncorrupted points $\text{conv}\{\phi_\gB(\vx) | \vx \in \gD_\gG\}$.
% \subsection{\textsc{Theoretical Guarantees}}

Theoretically, we can establish the following convergence guarantee for $\gmm$ :

\fcolorbox{black}{white}
{
    \begin{minipage}{0.95\linewidth}
    \begin{theorem}
        Suppose that, we are given, a set of $\alpha$-corrupted samples $\gD$ (\cref{def:corruption_model}), pretrained proxy model $\phi_\mB$, and an $\epsilon$ approx. $\gm(\cdot)$ oracle~\eqref{eq:gm}. Then, $\gmm$ guarantees that the mean of the selected $k$-subset $\bm{\mu}^\gS = \frac{1}{k} \sum_{\vx_i \in \gD_\gS}\vx_i$ converges to the neighborhood of $\bm{\mu}^\gG = \E_{\vx \in \gD_\gG}(\vx)$ at the rate $\gO(\frac{1}{k})$ such that:   
        \begin{equation}
        \label{equation:bound-z0-simplified}
            \E\bigg\|\bm{\mu}^\gS - \bm{\mu}^\gG\bigg \|^2\leq 
            \frac{8|\gD_\gG|}{(|\gD_\gG|-|\gD_\gB|)^2}\sum_{\vx \in \gD_\gG}\E\bigg\|\vx -\Mu^\gG \bigg\|^2 +\frac{2\epsilon^2}{(|\gD_\gG|-|\gD_\gB|)^2}
        \end{equation}
    \label{th:gm_match_cvg}
    \end{theorem}
\end{minipage}
}

This result suggest that, even in presence of $\alpha$ corruption, the proposed algorithm $\gm$ Matching converges to a neighborhood of the true mean, where the neighborhood radius depends on two terms -- the first term depend on the variance of the uncorrupted samples and the second term depends on how accurately the $\gm$ is calculated. Consequently, we say that $\gm$ Matching achieves the optimal breakdown point 1/2. The detailed proofs are provided in~\cref{sec:appendix}.  

% compute the discrepancy between the empirical distribution of the current samples and the target distribution; and chooses the next sample that most reduces this discrepancy, adding one sample at a time.
% set of random samples from $\gD$; compute the discrepancy between the empirical distribution of the current samples and the target distribution; and chooses the next sample that most reduces this discrepancy, adding one sample at a time, until the desired number of samples is reached or the discrepancy falls below a certain threshold. Note that, by converting the observed moments into a sequence of pseudo samples, herding diverges from the usual approach of first learning the joint distribution (which is often intractable) and then sampling from that model (which is prone to local mode entrapment). 

% More formally, suppose we are given a set of samples $\gX = \{\vx_i \in \sR^d \sim p(\rx)\}_{i=1}^N$ from the target distribution; and access to a foundation kernel $\phi_\gB(\cdot)$; then with some suitably chosen weight vector $\vtheta_0 =\phi_\mB(\vx_0 \in \gX) \in \sR^p $ Byzantine Robust Herding repeatedly performs the following updates until convergence:
% \begin{flalign}
%     \vx_{t+1} &:= \argmax_{\vx \in \gX} \; \langle\vtheta_t, \phi_\mB(\vx)\rangle\\
%     \vtheta_{t+1} &:= \vtheta_t + \textsc{Gm}(\phi_\mB(\vx)) - \phi_\mB(\vx_{t+1})
% \end{flalign}
% Note that this is simply performing a gradient ascent update along the 

% Intuitively, this mimics a weakly chaotic non linear dynamical system over the parameter space~\citep{welling2012herding}. 

% \textcolor{red}{
% * Use some sort of entropy formulation to characterize diversity. (ISD)
% \\
% * Equivalent moment matching objective. (ISD)
% }


  



==> NeuRips-2024/problem_setup.tex <==
Given a set of observations, 
%$\gD$, 
data pruning strategies aim to select a subset; such that  training a parametric model
% $f_\mtheta(\cdot)$ 
on the subset, yields (approximately) similar generalization performance as training on the entire dataset.
%$\gD$.  
However, this paper considers the setting where the training data
% $\gD$ 
is generated via an $\alpha$-corrupted generation process (\cref{def:corruption_model}). 
%%%%%%%%%%%%%%%%%%%%%%%

\fcolorbox{black}{white}%{LightCyan}
{
    \begin{minipage}{0.95\linewidth}
        \begin{definition}[{\bf $\alpha$-corrupted generation process}]
        \label{def:corruption_model}
            Given $\psi \in [0, \frac{1}{2})$ and a set of observations from the original distribution of interest, an adversary is allowed to \textbf{inspect} all the samples and \textbf{arbitrarily} perturb up to $\psi$ fraction of them. We refer to a set of samples $\gD = \gD_{\gG} \cup \gD_{\gB}$ generated through this process as $\alpha$-corrupted where, $\alpha:=|\gD_{\gB}|/ |\gD_{\gG}|  = \frac{\psi}{1 - \psi}< 1$. $\gD_{\gB}$ and $\gD_{\gG}$ denote the sets of corrupt and clean samples.
        \end{definition}
    \end{minipage}
}

%%%%%%%%%%%%%%%%%%%%%%%
Given such an $\alpha$-corrupted~\footnote{
    This strong corruption model is often referred to as the Gross Contamination Framework~\citep{diakonikolas2019recent}. It also generalizes the popular Huber Contamination Model~\citep{huber1992robust} as well as the notorious Byzantine Corruption Framework~\citep{lamport1982byzantine}.
} set of observations $\gD = \gD_{\gG} \cup \gD_{\gB} = \{(\vx_i, y_i) \in \sR^d \times \gY\}_{i=1}^N$, the goal of {\bf robust data pruning} is thus to judiciously select a subset $\gD_\gS \subseteq \gD$
 %of cardinality $ 0 < |\gS| \leq |\gD|$
; that {\em encapsulates the comprehensive statistical characteristics of the underlying clean (uncorrupted) distribution induced by subset $\gD_{\gG}$ without any a-priori knowledge about the corrupted samples}. 

Note that, allowing the noisy samples to be {\bf arbitrarily corrupted} enables us to generalize many important robustness scenarios; including \textbf{corrupt features, label noise} and {\bf adversarial attacks}.

% Needless to say, identifying sample importance is an ill-posed problem without some notion of similarity among the samples. Thus, we further assume access to a proxy encoder $\phi_\mB(\cdot): \sR^d \to \gH \in \sR^k$ that maps the features to a separable Hilbert space equiped with inner product. Intuitively, this simply means that the embedding space of the encoder fosters proximity of semantically similar examples, while enforcing the separation of dissimilar ones -- a property often satisfied by even off-the-shelf pretrained foundation models~\citep{hessel2021clipscore, sorscher2022beyond}. We refer the reader to~\cref{sec:exp}, where we investigate several choices for the proxy model.

% Note that, in addition to encoder $\phi(\cdot)$ gradient / uncertainty based sampling would require a linear layer $\vv : \sR^p \to |\gY|$, trained to map the embeddings to the appropriate label space. Clearly, this requires training on the original distribution which itself be problematic from the corrupted data, thus limiting the practical applicability of such methods.

% Given a set of observations $\gX$, and a pretrained proxy model $\phi_{\gB}(\cdot)$ 
% % e.g. CLIP~\citep{radford2021learning}, Llama2
% we aim to develop data pruning (also referred to as coreset selection, data filtering) strategies that judiciously select a subset (often referred to as a coreset) $\gS \subseteq \gX$ encapsulating the comprehensive statistical characteristics of the larger dataset. However, we are in the setting where a fraction of the training data can be arbitrarily corrupted. In particular, we consider the strong {\bf Gross Contamination Framework}~\citep{diakonikolas2019recent} (\cref{def:corruption_model}), that generalizes the popular {\bf Huber Contamination Model}~\citep{huber1992robust} as well as the notorious Byzantine Corruption Framework~\citep{lamport1982byzantine}.

% \begin{definition}
% [{\bf $\alpha$ corrupted generation process}]
% \label{def:corruption_model}
% Given $0 \leq \psi < \frac{1}{2}$ and a set of observations $\gX$, the adversary is allowed to \textbf{inspect} all the samples and {\bf arbitrarily} perturb up to $\psi |\gX|$ of them. In other words, the training dataset $\gX = \gX_{\gG} \cup \gX_{\gB}$, where $\gX_{\gB}$ and $\gX_{\gG}$ are the sets of corrupt and good samples. We interchangeably, refer to a set of samples generated through this process as $\alpha$-corrupted where $\alpha:=|\gX_{\gB}|/ |\gX_{\gG}|  = \frac{\psi}{1 - \psi}< 1$.
% \end{definition}

==> NeuRips-2024/rel_work.tex <==
% \input{plots/toy/fig.toy-corr=45}
% At its core, data pruning strategies 
At a high level, data pruning strategies leverage the concentration property of the feature space of to select samples based on some criterion over similarity measure between embeddings. Existing algorithms can be broadly divided into two categories: 

{\bf Importance Scoring Approach :}
The most popular set of approaches, possibly because of simplicity, rely on assigning an importance score to each sample. It stems from works in importance sampling, active learning.


{\bf Set Cover Approach :} One set of approaches~\citep{xia2022moderate, joshi2023data, sorscher2022beyond} : calculate the importance score of a sample in terms of the distance from the centroid of its corresponding class marginal 
% $d(\vx_i, y_i) = \| \phi_\mB(\vx_i) - \bm{\mu}_i \|_2^2 : \forall (\vx_i, y_i) \in \gD$ where, $\bm{\mu}_y = \frac{\sum_{(\vx_i, y_i) \in \gD}\1(y_i = y)\phi_\mB(\vx_i)}{\sum_{(\vx_i, y_i) \in \gD}\1(y_i = y)} : \forall y \in \gY$. 
In particular, samples closer to the centroid are considered most prototypical (easy) and those far from the centroid are treated as least prototypical (hard). It is worth noting that the distance-based score is closely related to the uncertainty / gradient based score. Samples close (far away) to the class centroid are often associated with smaller (larger) gradient norm and higher (lower) uncertainty~\citep{paul2021deep, sorscher2022beyond, xia2022moderate}.

Core-set selection methods have found widespread applications across several machine learning problems such as low resource training, active learning, continual learning, neural architecture search and model compression~\citep{ye2020good, liu2019metapruning, agarwal2005geometric, chen2020storage, he2019filter, li2019learning, maalouf2020deep} to name a few.

% In this work we will primarily focus on the using coreset selection approaches to improve the efficiency of training large scale machine learning models. 
% Our problem setting is described as follows: 
% At a high level, these methods aim to identify a representative subset (can be weighted) of the training data such that the subset approximates the joint distribution of the entire training dataset~\citep{welling2009herding, chen2010super}. The initial motivation of finding such subset was to be able to train ML models on the selected subset such that the resulting model generalizes equally well as the model trained on the whole dataset, while requiring an order of magnitude less compute resources~\citep{mirzasoleiman2020coresets}. 

At a high level all the data pruning approaches rely on defining some {\bf pruning metrics} and rank the training samples based on the scores and retain a fraction of them as representative samples (super samples), used for training the downstream model.  

% \paragraph{Supervised Coreset selection}
Most of the data pruning metrics require label information to compute ranking score. Typically they train the model $f$ for a pre-decided number of iterations $T_C$ using the whole dataset to select core-set using the trained model. 
% \paragraph{Geometry Based Methods.}

{\bf Geometry Based Methods.} Geometry based approaches rely on the key idea that samples that are close to each other in the feature space tend to have similar semantic properties and often redundant. For example, kernel herding methods~\citep{welling2009herding, chen2010super} select data points based on the distance between the coreset center and original dataset center in the feature space. They incrementally and greedily adds one sample each time into the coreset that can minimize distance between two centers. On the other hand k-center greedy approaches try to solve the mini-max facility location problem~\citep{farahani2009facility}. The problem is NP hard and thus solved using k-center greedy algorithm~\citep{agarwal2020contextual, sener2018active, sinha2020small}.  

{\bf Uncertainty Based Methods.}
These methods argue that samples with lower confidence are harder and may have a
greater impact on model optimization than those with higher confidence and thus should be included in the core-set. Thus, they use the confidence or other metrics that are function of confidence such as entropy, margin to compute pruning score~\citep{coleman2019selection}. 
% We first benchmark different core-set selection selection algorithms on three popular use cases: data efficient ML training, active learning and continual learning. In rest of this section we describe the use cases, tasks and experimental details in more detail.  

{\bf Gradient Based Methods.}
~\citep{mirzasoleiman2020coresets, killamsetty2021grad, killamsetty2021retrieve} try to find a subset of data points via greedy approximation such that the gradient computed on this subset closely follows the gradient of the entire dataset.   

{\bf Selection via proxy}
It is often observed that the accurate coreset selection algorithms itself are expensive thus dwarfing the benefit.~\citep{coleman2019selection} propose to use a smaller model $f_C$ instead of using the original model $f$ for the coresert selection iterations. The intuition is that the solutions are highly correlated to that obtained via $f$.

{\bf Unsupervised Coreset selection}
While, there has been several supervised coreset selection approaches, only a handful of approaches exits that do not require labeled data to compute the pruning score. For example, ~\citep{sorscher2022beyond} try to find cluster centers on the contrastive representation space; ~\citep{ju2022extending} directly uses the correlation between samples computed using infoNCE style loss to find coresets. 

While these methods are closely related to our setting, but note that they unsupervised approaches for coreset selection to improve efficiency of downstream supervised training. Whereas, our setting is to instead explore core-set selection strategies to improve the efficiency of self supervised learning while retaining the quality of produced representations (embeddings).  

Closest to our setting is ~\citep{robinson2020contrastive}, that uses uncertainty based approaches directly on the contrastive loss during contrastive training to identify hard negatives and get rid of easy negatives and show faster convergence - however, note that at each iterations they still need to compute contrastive loss on all the samples in the batch to identify hard negatives implying their per iteration cost is not improved.  




==> NeuRips-2024/scoring_dist_dev.tex <==
% \input{plots/toy/fig.toy_mean-estimation}
% Consider the problem of learning to approximate a continuous probability distribution function (PDF) $p_\gG(\rx)$ from a set of finite samples generated via $\alpha$-corruption~(\cref{def:corruption_model}) i.e. we only have access to 
% In particular, we focus on herding~\citep{welling2009herding, chen2010parametric, welling2010statistical} style algorithms that embody deterministic processes with infinite memory.

% \input{plots/toy/fig.toy_mean-estimation}
% \input{plots/toy/fig.toy-corr=45}
\input{plots/toy/fig.toy-corr=0}
\input{plots/toy/fig.toy-corr=20}
\input{plots/toy/fig.toy-corr=40}
\input{plots/toy/fig.toy-corr=45}
We begin by analyzing the robustness of existing data pruning algorithms under the strong gross contamination framework via breakdown point analysis~\citep{donoho1983notion} -- a common method to assess the resilience of an estimator. 

\fcolorbox{black}{white}
{
    \begin{minipage}{0.95\linewidth}
    \begin{definition}[{\textbf{Breakdown Point}}]
    \label{def:breakdown_point}
        The breakdown point of an estimator is defined as the smallest fraction of contaminated data that can cause the estimator to result in arbitrarily large errors. An estimator with a high breakdown point is considered robust because it can handle a larger amount of contamination before failing. In the context of Definition \ref{def:corruption_model} we say an estimator has \textbf{ optimal breakdown point 1/2} if it is robust in presence of $\alpha$-corruption 
        $\forall \; \alpha < 1$. 
    \end{definition}
% \begin{lemma}
%     No importance scoring criterion that samples relative to the class centroid, can tolerate a single grossly corrupted sample
% \end{lemma}
\end{minipage}
}

Score based pruning algorithms determine importance using similarity measures relative to the corresponding class centroid. For instance, consider the popular importance score:
\begin{flalign}
    d(\vx_i, y_i) = \| \vx_i - \bm{\mu}_y \|_2^2 : \forall (\vx_i, y_i) \in \gD
\end{flalign}
where, $\bm{\mu}_y$ denotes the class centroid , defined as:
\begin{flalign}
    \bm{\mu}_y = \frac{\sum_{(\vx_i, y_i) \in \gD}\1(y_i = y)\vx_i}{\sum_{(\vx_i, y_i) \in \gD}\1(y_i = y)} : \forall y \in \gY
\end{flalign} 
In the ideal setting, given a batch of i.i.d samples $\bm{\mu}_y = \bm{\mu}_y^\gG =\E_{\vx \sim \gD_\gG}(\vx)$. However, the presence of even a single grossly corrupted sample can cause the centroid estimate to deviate arbitrarily from the true mean. Consider a single grossly corrupt sample $(\vx_i^\gB, y_i)$ such that : 
\begin{flalign}
    \vx_i^\gB = {\sum_{(\vx_i, y_i) \in \gD}\1(y_i = y)}\bm{\mu}_y^\gB - \sum_{(\vx_i, y_i) \in \gD \setminus (\vx_i^\gB, y_i)}\1(y_i = y)\vx_i
    \label{eq:adv}
\end{flalign}
resulting in shifting the estimated centroid $\Delta\bm{\mu}_y = \bm{\mu}_y^\gB -\bm{\mu}_y^\gG$ 
% This would completely distort the score distribution
% Thus, forcing the data selection algorithm to select samples around some adversarially chosen $\tilde{\bm{\mu}}_y$.
%, which can be arbitrarily away from the true mean. 
\begin{lemma}
    A single gross corrupted sample~\eqref{eq:adv} causes the importance scores to deviate arbitrarily:
    \begin{flalign}
        \Delta d(\vx_i, y_i) = \|\Delta \bm{\mu}_y\|^2 - 2\bigg(\vx_i - \bm{\mu}_y^\gG\bigg)^T \Delta \bm{\mu}_y
    \end{flalign}
    Implying, these methods yield the {\bf lowest possible asymptotic breakdown of 0}.
    \label{lemma:score_dist_dev}
\end{lemma}
Similarly, under the same corruption, moment matching based methods, would to find subsets such that centroid of the subset is closely aligned to the perturbed centroid implying a bias $\gO(\Delta \bm{\mu}_y)$. Thus, moment matching based methods also has the {\bf asymptotic breakdown of 0}.
\cref{fig:toy-corr=45},\ref{fig:toy-mean-estimation} validates these theoretical implications.
% e.g. Kernel Herding~\citep{chen2010super, welling2009herding}, CRAIG~\citep{mirzasoleiman2020coresets}
% GradMatch~\citep{killamsetty2021grad} would be encouraged find subset $\gS \subseteq \gD$ such that $\E(\gS) = \tilde{\bm{\mu}}_y$ which can be arbitrarily far from the true underlying moment. 

==> NeuRips-2024/tables/tab-noisy-35.tex <==
\begin{table*}
    \footnotesize
    \centering
    \begin{tabular}{lccccc}
        \toprule
        
        & \multicolumn{2}{c}{\bf CIFAR-100 (Label noise)} 
        & \multicolumn{2}{c}{\bf Tiny ImageNet (Label noise)} 
        & \\
        \cmidrule(r){2-3} 
        \cmidrule(r){4-5} 
        {\bf Method / Ratio } 
        & 20\% 
        & 30\% 
        & 20\% 
        & 30\% 
        & {\bf Mean $\uparrow$} 
        \\
        \midrule
        Random 
        & 24.51$\pm$1.34 
        & 32.26$\pm$0.81 
        & 14.64$\pm$0.29 
        & 19.41$\pm$0.45 
        &
        \\
        Herding 
        & 29.42$\pm$1.54 
        & 37.50$\pm$2.12 
        & 15.14$\pm$0.45 
        & 20.19$\pm$0.45 
        & 
        \\
        Forgetting 
        & 29.48$\pm$1.98 
        & 38.01$\pm$2.21 
        & 11.25$\pm$0.90 
        & 17.07$\pm$0.66 
        & 
        \\
        GraNd-score 
        & 23.03$\pm$1.05 
        & 34.83$\pm$2.01 
        & 13.68$\pm$0.46 
        & 19.51$\pm$0.45 
        & 
        \\
        EL2N-score 
        & 21.95$\pm$1.08 
        & 31.63$\pm$2.84 
        & 10.11$\pm$0.25 
        & 13.69$\pm$0.32 
        & 
        \\
        Optimization-based 
        & 26.77$\pm$0.15 
        & 35.63$\pm$0.92 
        & 12.37$\pm$0.68 
        & 18.52$\pm$0.90 
        & 
        \\
        Self-sup.-selection 
        & 23.12$\pm$1.47 
        & 34.85$\pm$0.68 
        & 11.23$\pm$0.32 
        & 17.76$\pm$0.69 
        &
        \\
        Moderate-DS 
        & 28.45$\pm$0.53 
        & 36.55$\pm$1.26 
        & 15.27$\pm$0.31 
        & 20.33$\pm$0.28 
        & 
        \\
        {\bf $\gm$ Matching}
        & {\bf 43.33$\pm$ 1.02}
        & {\bf 58.41$\pm$ 0.68}
        & {\bf 23.14$\pm$ 0.92} 
        & {\bf 27.76$\pm$ 0.40}
        & 
        \\
        \bottomrule
    \end{tabular}
    \caption{35\% Label Noise}
    \label{tab:label-noise-0.35}
\end{table*}


==> figs_meta/algo_diag.tex <==
\begin{figure}[]
\includegraphics[width=\textwidth]{figs_meta/algo_diag.png} 
% \subfloat[\footnotesize Spearman Rank Correlation]{\includegraphics[width=0.6\textwidth]{figs/proxy_epochs_resnet18_cifar10_corr.png}\label{fig:lp_nP}}
\caption{\footnotesize {\bf tsne visualization of unsupervised coreset selection on $\ell_2$ hypersphere framework}: {\em The unlabeled training samples from CIFAR-10 are projected to the embedding space using an off-the-shelf pretrained ResNet18 encoder (trained for 300 epochs) followed by the coreset selection on the embedding space using the proposed pruning metric leveraging the geomtric property of the samples}}
\label{figure:punce_ablation}
\end{figure}

==> figs_meta/cifar_table.tex <==
\begin{table*}[]
\centering
\footnotesize 
% \setlength{\tabcolsep}{4 pt}
% \resizebox{\textwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
Dataset  
& $f_p(\cdot)$
& Coreset Size
& Uniform
% & DCL
& Hard
& Hard+Center
\\ \midrule \midrule 
\multirow{5}{2 cm}{\centering CIFAR 10} 
& \multirow{5}{2 cm}{\centering ResNet18 \\(300 epochs)} 
& 5\%    
& $\textcolor{red}{- 18.66\%}$          
& $\textcolor{red}{- 17.56\%}$        
& $\textcolor{red}{- 11.18\%}$    
\\ 
&
&10\%    
& $\textcolor{red}{- 13.24\%}$          
& $\textcolor{red}{- 12.59\%}$       
& $\textcolor{red}{-  6.38\%}$    
\\
&
&30\%    
& $\textcolor{red}{- 8.06\%}$          
& $\textcolor{red}{- 4.80\%}$       
& $\textcolor{red}{- 1.02\%}$     
\\
&
&50\%    
& $\textcolor{red}{- 3.99\%}$         
& $\textcolor{red}{- 0.64\%}$       
& $\textcolor{green}{+ 0.13\%}$     
\\
&
&70\%    
& $\textcolor{red}{- 2.51\%}$              
& $\textcolor{green}{+ 0.17\%}$        
& $\textcolor{green}{+ 0.29\%}$     
\\\bottomrule
\end{tabular}
%}
\caption{ResNet-18 on CIFAR 10 with coreset
results denote relative improvement (or regression) with 
respect to the baseline i.e., training on the entire training 
on entire training data.
}
\label{tab:cifar10_coreset}
\end{table*}

==> figs_meta/coreset_results.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
% \vspace*{-2 em}
  \begin{center}
    \includegraphics[width=0.4\textwidth]{figs_meta/kMeans_hard_centers_300.png}
  \end{center}
 \caption{\footnotesize Unsupervised coreset selection generalization performance while training ResNet18 on CIFAR10 with varying size of coreset. We use a 300 epoch trained ResNet18 as proxy model for the coreset selection.}
 \label{fig:coreset_results}
% \vspace*{-1 em}
\end{wrapfigure}

==> figs_meta/corr_proxy.tex <==
\begin{figure}[]
\centering
\subfloat[\footnotesize Proxy Models]{\includegraphics[width=0.3\textwidth]{figs_meta/infoNCE_epochs.png} \label{fig:cls_nP}}
\subfloat[\footnotesize Spearman Rank Correlation]{\includegraphics[width=0.4\textwidth]{figs_meta/proxy_epochs_resnet18_cifar10_corr.png}\label{fig:lp_nP}}
\subfloat[\footnotesize Selected coreset e-300]{\includegraphics[width=0.3\textwidth]{figs_meta/kmeans_coreset_1k.png}\label{fig:lp_nP}}
\caption{Comparing proxy models}
\label{figure:proxy_ablation}
\end{figure}

==> figs_meta/kmeans_manifold.tex <==
%\begin{wrapfigure}{r}{0.48\textwidth}
% \vspace*{-2 em}
%   \begin{center}
%     \includegraphics[width=0.48\textwidth]{figs/kmeans_manifold.png}
%   \end{center}
%  \caption{\footnotesize k-means clustering on the unit norm hypersphere on a synthetic dataset to identify super samples and hard examples.}
%  \label{fig:kmeans_manifold}
% \vspace*{-2.5 em}
% \end{wrapfigure}
\begin{figure}[]
\centering
\subfloat[\footnotesize Contrastive Learning]{\includegraphics[width=0.45\textwidth]{figs_meta/contrastive_learning.png} \label{fig:cl_hyp}}
\subfloat[\footnotesize k-means on hypersphere manifold]{\includegraphics[width=0.45\textwidth]{figs_meta/kmeans_manifold.png}\label{fig:cs_hyp}}
\caption{Comparing proxy models}
\label{figure:contrastive_hypersphere}
\end{figure}


==> figs_meta/lp_ft.tex <==
\begin{figure}[]
\centering
\includegraphics[width=0.8\textwidth]{figs_meta/LP_FT.png}
\caption{Transfer Learning Strategies}
\label{figure:contrastive_hypersphere}
\end{figure}

==> figs_meta/ssl_data_scaling_law.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
%\vspace*{-2 em}
  \begin{center}
    \includegraphics[width=0.38\textwidth]{figs_meta/infoNCE_scaling_law.png}
  \end{center}
 \caption{\footnotesize {\bf Data scaling law for contrastive training}: Comparing generalization result for training ResNet-18 only on a random subset ($0 < k \leq 1$ fraction for varying k) of CIFAR 10 data.}
 \label{fig:scaling_ssl}
% \vspace*{-1 em}
\end{wrapfigure}

==> icml/SSL_pretrain.tex <==
\subsection*{Background}

{\bf Baselines: } 
\begin{itemize}
    \item Random Sampling $\gO(N)$
    \item \citep{sorscher2022beyond}
    \item \citep{joshi2023data}
\end{itemize}

\subsection*{Neural Scaling laws for CURL}
\input{icml/results/tab.scaling_law_ssl}

\subsection*{Beating Scaling Law: Importance Sampling}
\input{icml/results/tab.clustdist_ablation_k}

\paragraph{Mixing hard examples :} 
Easy examples are important during the beginning of training or when the coreset size is small. Coreset Selection - training from scratch using hard is bad - easy is better. We use a ResNet-18 trained using SimCLR on CIFAR-10 for 49 epochs as proxy model to select coreset. Then we train a ResNet-18 from scratch using the hard and easy examples only.  

Hard examples are useful later or when the coreset size is larger. Continual learning w hard is better than easy. We use a ResNet-18 trained using SimCLR on CIFAR-10 for 49 epochs as proxy model to sele3ct coreset. Then we continue training the ResNet-18 using the hard and easy examples only.   

\input{icml/results/tab.compare_unsup_metric}


\begin{table*}[ht]
\centering
\begin{tabular}{ccccccc}
\hline
\multirow{2.5}{*}{\bf Proxy Model}
&\multirow{2.5}{*}{\bf Hard Mixing ($\lambda$)}
& \multicolumn{5}{c}{\bf Coreset Fraction ($\gamma$)}
\\\cmidrule(lr){3-7}
&
&\textbf{5\%} 
&\textbf{10\%} 
&\textbf{30\%} 
&\textbf{50\%} 
&\textbf{70\%} 
\\
\hline\hline 
{\bf -} 
& -
& 65.34
& 71.88
& 80.99
& 84.50 
& 86.07 
\\
\\
\multirow{7}{*}{\bf ResNet18 (50)}
& 0.0
&\textcolor{blue}{\bf 66.85} 
&72.07 
&\textcolor{magenta}{79.83} 
&\textcolor{magenta}{83.28} 
&\textcolor{magenta}{86.04} 
\\
& 0.1
& 66.49
& 72.42
& 79.94
& 83.37
& 86.26
\\
& 0.3
& 66.09
& \textcolor{blue}{\bf 72.54}
& 80.35
& 84.01
& 86.43
\\
& 0.5
& 65.57
& \textcolor{blue}{72.48}
& 81.00
& 84.34
& 86.38
\\
& 0.7
& 65.29
& 71.84
& \textcolor{blue}{\bf 81.45}
& \textcolor{blue}{84.38}
& 86.57
\\
& 0.9
& 63.84
& 71.09
& 80.53
& \textcolor{blue}{\bf 84.53}
& \textcolor{blue}{86.72}
\\
& 1.0
& \textcolor{magenta}{63.37} 
& \textcolor{magenta}{69.89} 
& \textcolor{blue}{81.13} 
& 84.34
& \textcolor{blue}{\bf 86.91} 
\\
\\
\multirow{7}{*}{\bf ResNet18 (100)}
& 0.0
& \textcolor{blue}{\bf 67.15}
& 72.81
& 
&
&
\\
& 0.1
& \textcolor{blue}{67.13}
& 72.95
& 
&
&
\\
& 0.3
& 66.91
& 73.04
& 
&
&
\\
& 0.5
& 66.29
& 72.60
& 
&
&
\\
& 0.7
& 65.49
& 71.82
& 
&
&
\\
& 0.9
& 64.97
& 70.62
& 
&
&
\\
& 1.0
& \textcolor{magenta}{63.43}
& \textcolor{magenta}{69.20}
& 
&
&
\\
\hline
\end{tabular}
\caption{{\bf Proxy Model Training:} Proxy Models used for importance sampling is also a ResNet-18 trained for (50, 100, 200, 400) epochs}
\label{tab.proxy_epoch}
\end{table*}


% {\bf Coreset}

% (random): (5\%) 65.34 ; (10\%) 71.88 ; (30\%) 80.99
% \\
% (easy-49): (5\%) {\bf 66.85} ; (10\%) {\bf 72.07} ; (30\%) 79.83
% \\
% (hard-49): (5\%) 63.37 ; (10\%) 69.89 ; (30\%) {\bf 81.13}






==> icml/generalization.tex <==
We assume access to a set family of stochastic label preserving transformations $t(\cdot)\sim \gT : \sR^d\to\sR^d$, such as color distortion, cropping, flipping, etc. We define the augmentation set $A(\vx)$ to be the set of all possible augmentations of an input $\vx$. We assume that: 
$\vx \in A(x)$ and the augmentations are class preserving i.e.
$A(C_k) \cap A(C_l) = \varnothing ,\; \forall k \neq l$.

\begin{definition}[{\bf($\sigma, \delta$) Augmentation}]~\cite{huang2023towards} bla bla   
\end{definition}

To simplify the analysis we consider a non-parametric nearest neighbor classifier to provide generalization guarantee on the downstream classification: 
\begin{flalign}
    F_{g_\mB}(\vx) = \argmin_{k \in [K]} \|g_\mB(\vx) - \bm{\mu}_k\|
\end{flalign}
Where, $\bm{\mu}_k = \E_{\vx_i \in C_k}\E_{\vx' \in A(\vx_i)} g_\mB(\vx')$ denote centroid of the embeddings of class $C_k$.
 
\begin{lemma}
    \cite{huang2023towards} The Nearest Neighbor Classifier $F_{g_\mB}(\cdot)$ can be formulated as a linear classifier:
    \begin{flalign*}
    F_{g_\mB}(\vx) 
    &= \argmin_{k \in [K]} \|g_\mB(\vx) - \bm{\mu}_k\| \\
    &= \argmax_{k \in [K]} \bigg( \bm{\mu}_k^Tg_\mB(\vx) - \frac{1}{2}\|\bm{\mu}_k\|^2\bigg)
    \end{flalign*}
    \label{lemma:NN_as_linear}
\end{lemma}
\begin{proof}
    Consider, $F_{g_\mB}(\vx) = k$, then $\forall l \in [K]$ : 
    \begin{flalign*}
        &\|g_\mB(\vx) - \bm{\mu}_k\|^2 \leq \|g_\mB(\vx) - \bm{\mu}_l\|^2 \\
        \implies &\bm{\mu}_k^T g_\mB(\vx) - \frac{1}{2}\|\bm{\mu}_k\|^2 \geq \bm{\mu}_l^T g_\mB(\vx) - \frac{1}{2}\|\bm{\mu}_l\|^2
     \end{flalign*}
Clearly, this is equivalent to a linear classifier :
\begin{flalign*}
    F_{g_\mB}(\vx) = \argmax_{k \in [K]}\bigg( \bm{\mu}_k^Tg_\mB(\vx) - \frac{1}{2}\|\bm{\mu}_k\|^2\bigg)
    \end{flalign*}
\end{proof}
Thus, we use the classification error rate of $F_{g_\mB}(\cdot)$ to bound the downstream classification performance.~\cref{lemma:NN_as_linear} suggest that also bounds the worst case performance of the linear classifier. 
\begin{flalign}
    err(F_{g_\mB}) = \sum_{k=1}^k P\bigg[F_{g_\mB}(\vx)) \neq k, \; \forall \vx \in C_k\bigg]
\end{flalign}

Given a dataset $\gX = \{\vx_i\}_{i=1}^n$ and access to a stochastic family of class preserving augmentation, our goal is to study $\epsilon$-coresets of the training data i.e. find subsets $\gX^s \subseteq \gX$ of size $\gamma|\gX|$ where $0 < \gamma \leq 1$ such that training on the subset with contrastive loss yields $\epsilon$ approximation of the downstream classification performance $err(F_{g_\mB})$.

\begin{definition}[\bf Augmentation distance]
    Augmentation distance between two samples in an augmentation set is defined as the minimum distance between all possible augmented views of the samples: 
    \begin{flalign}
    d_A(\vx_1, \vx_2) = \sup_{\vx_1\in A(\vx_1),\vx_2 \in A(\vx_2)}\bigg\|f(\vx_1) - f(\vx_2)\bigg\|
\end{flalign}
\end{definition}
Let, $S_\epsilon$ denote the set of samples with $\epsilon$-close representations among augmented data i.e :$S_\epsilon:= \bigg\{\vx \in \cup_{k=1}^K C_k : \forall \vx_1,\vx_2 \in A(\vx), \bigg\|f(\vx_1) - f(\vx_2)\bigg\| \leq \epsilon\bigg\}$. Further, we let $R_\epsilon(\gX) = P( \bar{S_\epsilon} )$ denote the probability of embeddings from the same class to have non-aligned augmented views.

~\citep{huang2023towards} shows for contrastive learning with infoNCE family of losses the following holds:
\begin{flalign}
    R_\epsilon(\gX) \leq \eta(\epsilon) \E_\vx \E_{\vx_1, \vx_2 \in A(\vx)}\bigg\|g_\mB(\vx_1) - g_\mB(\vx_2)\bigg\|
\end{flalign}

We can now derive this for any random coreset from $A(\vx)$. For class $k$ we have: 
\begin{flalign*}
    &R_\epsilon(\gX_k) \\
\leq& \eta(\epsilon) \E_\vx \E_{\vx_1, \vx_2 \in A(\vx)}\bigg\|\vz_1 - \vz_2\bigg\|\\
    =&\frac{\eta(\epsilon)}{n_k} \bigg( \sum_{i \in \gX_k^s}\E_{\vx_1, \vx_2 \in A(\vx)} \bigg\|\vz_1 - \vz_2\bigg\|\\
    &+ \sum_{i \in {\gX_k \setminus \gX_k^s}}\E_{\vx_1, \vx_2 \in A(\vx)} \bigg\|\vz_1 - \vz_2\bigg\|\bigg)\\
\leq& \frac{\eta(\epsilon)}{n_k} \bigg( \sum_{i \in \gX_k^s}d_A(\vx_1, \vx_2) + 2L \min_{j \in \gX_k^s}\sum_{i \in \gX_k^s} d_A(\vx_i, \vx_j)\bigg)
\end{flalign*}

==> icml/importance_sampling.tex <==
The backbone of data pruning is an unsupervised importance scoring metric. 

Given $N$ vectors $\{\vv_i \in \sR^d\}_{i=1}^N$, the task is to find $0 < \gamma \leq 1$ fraction of most important vectors based on some importance metric.

\citep{sorscher2022beyond, joshi2023data}
\subsection{AugAlign : Augmentation Alignment}
Label Preserving Distortions.

Role of Augmentation Quality 

Role of M



 



==> icml/intro.tex <==
Given a set of points $\sP$ in some metric space, coreset is defined as a representative subset $\sD$ that approximates $\sP$ with respect to some extent measure (e.g. objective function)~\citep{feldman2020core, agarwal2005geometric, muthukrishnan2005data, har2011geometric, feldman2011unified}. More formally, for a set of candidate queries $\sX$ and a measure function {\bf cost}$(\sP, x\in \sX)$, subset $\sD$ is referred to as an $\epsilon$-coreset of $\sP$ if $\forall x \in \sX$, {\bf cost}$(\sD, x)$ is an approximation of {\bf cost}$(\sP, x)$ up to a multiplicative factor of $1 \pm \epsilon$.

Core-set selection methods have found widespread applications across several machine learning problems such as low resource training, active learning, continual learning, neural architecture search and model compression~\citep{ye2020good, liu2019metapruning, agarwal2005geometric, chen2020storage, he2019filter, li2019learning, maalouf2020deep} to name a few.




{\bf Efficient Training:} Coreset Selection - Data Efficient Training / Fine-Tuning of foundation models.   

{\bf Better Generalization:} Continual Learning to improve generalization 

Vision:
(a) SSL Foundation model training,  
(b) FineTune SSL foundation model,

NLP: FineTuning a LLM on a fraction of data (DEFT)

MultiModal: Similar idea can be extended to multi-modal CLIP style settings instead of CLIP score. 

\input{icml/results/tab.coreset_complexity}

==> icml/rel_work.tex <==
Most of the data pruning metrics require label information to compute ranking score. Typically they train the model $f$ for a pre-decided number of iterations $T_C$ using the whole dataset to select core-set using the trained model. 
% \paragraph{Geometry Based Methods.}

{\bf A. Geometry Based Methods.} Geometry based approaches rely on the key idea that samples that are close to each other in the feature space tend to have similar semantic properties and often redundant. For example, kernel herding methods~\citep{welling2009herding, chen2010super} select data points based on the distance between the coreset center and original dataset center in the feature space. They incrementally and greedily adds one sample each time into the coreset that can minimize distance between two centers. On the other hand k-center greedy approaches try to solve the mini-max facility location problem~\citep{farahani2009facility}. The problem is NP hard and thus solved using k-center greedy algorithm~\citep{agarwal2020contextual, sener2018active, sinha2020small}.  

{\bf B. Uncertainty based approaches}
These methods argue that samples with lower confidence are harder and may have a
greater impact on model optimization than those with higher confidence and thus should be included in the core-set. Thus, they use the confidence or other metrics that are function of confidence such as entropy, margin to compute pruning score~\citep{coleman2019selection}. 
% We first benchmark different core-set selection selection algorithms on three popular use cases: data efficient ML training, active learning and continual learning. In rest of this section we describe the use cases, tasks and experimental details in more detail.  

{\bf C. Gradient based approaches}
~\citep{mirzasoleiman2020coresets, killamsetty2021grad, killamsetty2021retrieve} try to find a subset of data points via greedy approximation such that the gradient computed on this subset closely follows the gradient of the entire dataset.   

{\bf Selection via proxy}
It is often observed that the accurate coreset selection algorithms itself are expensive thus dwarfing the benefit.~\citep{coleman2019selection} propose to use a smaller model $f_C$ instead of using the original model $f$ for the coresert selection iterations. The intuition is that the solutions are highly correlated to that obtained via $f$.

{\bf Unsupervised Coreset selection}
While, there has been several supervised coreset selection approaches, only a handful of approaches exits that do not require labeled data to compute the pruning score. For example, ~\citep{sorscher2022beyond} try to find cluster centers on the contrastive representation space; ~\citep{ju2022extending} directly uses the correlation between samples computed using infoNCE style loss to find coresets. 

While these methods are closely related to our setting, but note that they unsupervised approaches for coreset selection to improve efficiency of downstream supervised training. Whereas, our setting is to instead explore core-set selection strategies to improve the efficiency of self supervised learning while retaining the quality of produced representations (embeddings).  

Closest to our setting is ~\citep{robinson2020contrastive}, that uses uncertainty based approaches directly on the contrastive loss during contrastive training to identify hard negatives and get rid of easy negatives and show faster convergence - however, note that at each iterations they still need to compute contrastive loss on all the samples in the batch to identify hard negatives implying their per iteration cost is not improved.

==> icml/results/tab.clustdist_ablation_k.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{cccccccc}
\hline
\multirow{2.5}{*}{\bf Metric}
&\multirow{2.5}{*}{\bf \# Clusters ($k$)}
&\multirow{2.5}{*}{\bf Sampling}
&\multicolumn{5}{c}{\bf Coreset Fraction ($\gamma$)}
\\\cmidrule(lr){4-8}
&
&
&\textbf{5\%} 
&\textbf{10\%} 
&\textbf{30\%} 
&\textbf{50\%} 
&\textbf{70\%} 
\\
\hline\hline 
Uniform
& -
& -
& \textcolor{blue}{65.34} 
& 71.88
& 80.99
& \textcolor{blue}{84.50} 
& 86.07 
\\
\\
\multirow{9}{*}{ClustDist}
& 5
& \multirow{4}{*}{Easy}
& 55.21
& 64.07
& 76.56
& 82.58
& 86.49
\\
& 10
& 
& 58.31
& 66.05
& 76.32
& 82.94
& 86.57
\\
& 50
&
& 58.90
& 65.53
& 77.09
& 83.89
& 86.46
\\
& 100
&
& 58.59
& 64.39
& 76.96
& 83.52
& 86.67
\\
\\
{\citep{sorscher2022beyond}}
& 5
& \multirow{4}{*}{Hard}
& 58.26
& 65.60
& 77.06
& 82.41
& 85.98
\\
& 10
& 
& 
& 
& 
& 
& 
\\
& 50
&
& 
& 
& 
& 
& 
\\
& 100
&
& 
& 
& 
& 
& 
\\
\\
\multirow{2}{*}{AugAlign ( M = 2 )}
& \multirow{2}{*}{-}
& Easy
& 66.85
& 72.07 
& 79.83 
& 83.28
& 86.04
\\
&
& Hard
& 63.37
& 69.89 
& 81.13 
& 84.34
& 86.91 
\\
\hline
\end{tabular}
\caption{{\bf Clustdist sensitivity to k :} Coresets-CIFAR10: SimCLR trained using ResNet-18 on CIFAR10 on (5, 10, 30, 50, 70)\% of full dataset {\bf Baseline (full): 88.46}. 
Proxy encoder $\Phi(\cdot) : \sR^d \to \sR^p$ used for importance sampling is also a ResNet-18 trained for 50 epochs on full CIFAR-10 training dataset}
\label{tab:clustdist_ablation_k}
\end{table*}

==> icml/results/tab.compare_unsup_metric.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{ccccccc}
\hline
\multirow{2.5}{*}{\bf Metric}
&\multirow{2.5}{*}{\bf Hard Mixing ($\lambda$)}
& \multicolumn{5}{c}{\bf Coreset Fraction ($\gamma$)}
\\\cmidrule(lr){3-7}
&
&\textbf{5\%} 
&\textbf{10\%} 
&\textbf{30\%} 
&\textbf{50\%} 
&\textbf{70\%} 
\\
\hline\hline 
{\bf uniform} 
& -
& \textcolor{blue}{65.34} 
& 71.88
& 80.99
& \textcolor{blue}{84.50} 
& 86.07 
\\
\\
\multirow{7}{*}{\bf AugAlign ( M = 2 )}
& 0.0
&\textcolor{blue}{\bf 66.85} 
&72.07 
&\textcolor{magenta}{79.83} 
&\textcolor{magenta}{83.28} 
&\textcolor{magenta}{86.04} 
\\
& 0.1
& 66.49
& 72.42
& 79.94
& 83.37
& 86.26
\\
& 0.3
& 66.09
& \textcolor{blue}{\bf 72.54}
& 80.35
& 84.01
& 86.43
\\
& 0.5
& 65.57
& \textcolor{blue}{72.48}
& 81.00
& 84.34
& 86.38
\\
& 0.7
& 65.29
& 71.84
& \textcolor{blue}{\bf 81.45}
& 84.38
& 86.57
\\
& 0.9
& 63.84
& 71.09
& 80.53
& \textcolor{blue}{\bf 84.53}
& \textcolor{blue}{86.72}
\\
& 1.0
& \textcolor{magenta}{63.37} 
& \textcolor{magenta}{69.89} 
& \textcolor{blue}{81.13} 
& 84.34
& \textcolor{blue}{\bf 86.91} 
\\
\\
\multirow{7}{*}{\bf clustdist (k=10)}
& 0.0
& 58.31
& 66.05
& 76.32
& 82.94
& 86.57
\\
& 0.1
&
&
& 
& 
& 
\\
& 0.3
&
&
& 
& 
& 
\\
& 0.5
&
&
& 
& 
& 
\\
& 0.7
&
&
& 
& 
& 
\\
& 0.9
&
&
& 
& 
& 
\\
& 1.0
&
&
& 
& 
& 
\\
\\
\multirow{7}{*}{\bf clustdist (k=100)}
& 0.0
& 58.59
& 64.39
& 
& 
& 
\\
& 0.1
& 
&
& 
& 
& 
\\
& 0.3
&
&
& 
& 
& 
\\
& 0.5
&
&
& 
& 
& 
\\
& 0.7
&
&
& 
& 
& 
\\
& 0.9
&
&
& 
& 
& 
\\
& 1.0
&
&
& 
& 
& 
\\
\hline
\end{tabular}
\caption{{\bf Unsupervised Pruning Metrics:} Coresets-CIFAR10: SimCLR trained using ResNet-18 on CIFAR10 on (5, 10, 30, 50, 70)\% of full dataset {\bf Baseline (full): 88.46}. 
Proxy Models used for importance sampling is also a ResNet-18 trained for 50 epochs on full CIFAR-10 training dataset}
\label{tab:compare_algos}
\end{table*}

==> icml/results/tab.coreset_complexity.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{cc}
\hline
\textbf{Algorithm} 
&\textbf{Coreset Computation} 
\\
\hline\hline
\citep{sorscher2022beyond}
& $\gO\Bigg(\bigg( 1 + \textcolor{blue}{\tau k}d + \gamma \log(\gamma N)\bigg)N\Bigg)$
\\
\cite{joshi2023data}
& $\gO\Bigg(\bigg( 1 + \textcolor{blue}{\tau k}d + \gamma \log(\gamma N)\bigg)N + \textcolor{blue}{\sum_{i=1}^kN_i^2 d}\Bigg)$
\\
AugAlign (This work)
&$\gO\Bigg(\bigg( 1 + d + \gamma \log(\gamma N)\bigg)N\Bigg)$
\\
\hline
\end{tabular}
\caption{{\bf Computational Complexity of Unsupervised Data Pruning:} Given $N$ vectors $\{\vv_i \in \sR^d\}_{i=1}^N$, the task is to find $0 < \gamma \leq 1$ fraction of most important vectors based on some importance metric. We compare the time complexity of existing unsupervised importance metrics with the proposed AugAlign metric. Prior work~\citep{sorscher2022beyond, joshi2023data} rely on clustering the vectors in order to compute the scores ; $\tau \geq 1$ is the number of iterations for clustering, $k \geq 1$ denotes the number of clusters and $N_i$ is the number of samples in cluster indexed by $i$. For large scale datasets clustering can itself become the computational bottleneck. AugAlign improves over both the methods - the savings become are more significant in large scale settings.}
\label{tab:coreset_complexity}
\end{table*}

==> icml/results/tab.scaling_law_ssl.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{cccccccc}
\hline
\multirow{2.5}{*}{\bf Dataset}
&\multirow{2.5}{*}{\bf Model}
& \multicolumn{5}{c}{\bf Data Fraction ($\gamma$)}
\\\cmidrule(lr){3-8}
&
&\textbf{5\%} 
&\textbf{10\%} 
&\textbf{30\%} 
&\textbf{50\%} 
&\textbf{70\%} 
&\textbf{100\%} 
\\
\hline\hline 
\multirow{3}{*}{\bf CIFAR 10}
&{\bf ReseNet-18} 
& 65.34
& 71.88
& 80.99
& 84.50 
& 86.07 
& 88.46
\\
&{\bf ReseNet-34} 
& 65.82
& 72.55
& 81.52
& 85.19 
& 87.62
& 89.71
\\
&{\bf ReseNet-50} 
& 67.71
& 74.41
& 83.13
& 86.49
& 88.58
& 90.41
\\
\hline
\end{tabular}
\caption{{\bf Scaling Law for SSL:} SimCLR trained on (5, 10, 30, 50, 70)\% of full dataset sampled uniformly at random from the training set.}
\label{tab:scaling_law}
\end{table*}

==> plots/CIFAR-10-Scratch-Label-Noise/fig.tex <==
% \setlength{\abovecaptionskip}{2pt}  % Set this globally just after loading your packages
% \setlength{\intextsep}{-1pt}         % Reduce space above and below the floats
\begin{figure} 
\centering
\subfloat[\textsc{No Corruption}]
{\includegraphics[width=0.33\textwidth]
{plots/CIFAR-10-Scratch-Label-Noise/psi=0.pdf}}
\subfloat[\textsc{20\% Symm Label Noise}]
{\includegraphics[width=0.33\textwidth]
{plots/CIFAR-10-Scratch-Label-Noise/psi=20.pdf}}
\subfloat[\textsc{40\% Symm Label Noise}]
{\includegraphics[width=0.33\textwidth]
{plots/CIFAR-10-Scratch-Label-Noise/psi=40.pdf}}

\caption{ResNet-18 (random) is trained on CIFAR10. Proxy: ResNet18 pretrained on ImageNet-1k.}
\label{fig:CIFAR10-Scratch-Label-Noise}
\end{figure}

==> plots/CIFAR-10-Scratch-Label-Noise/main-fig.tex <==
\begin{figure*}[t]
\centering
\subfloat[\textsc{No Corruption}]
{\includegraphics[width=0.3\textwidth]
{plots/CIFAR-10-Scratch-Label-Noise/psi=0.pdf}}
\subfloat[\textsc{20\% Symm Label Noise}]
{\includegraphics[width=0.3\textwidth]
{plots/CIFAR-10-Scratch-Label-Noise/psi=20.pdf}}
\subfloat[\textsc{40\% Symm Label Noise}]
{\includegraphics[width=0.3\textwidth]
{plots/CIFAR-10-Scratch-Label-Noise/psi=40.pdf}}

\caption{
\footnotesize
{\bf Domain Transfer ( ImageNet-1k $\rightarrow$ CIFAR-10 ) Proxy :} CIFAR10, corrupted with label noise is pruned using a (proxy) ResNet-18 pretrained on ImageNet-1k. A ResNet-18 is trained from scratch on the subset. We compare our method \textsc{GM Matching} with geometric pruning baselines: \textsc{Uniform}, \textsc{Easy},\textsc{Hard}, \textsc{Moderate}, \textsc{Herding}.}
\label{fig:main-cifar-vanilla}
\end{figure*}

==> plots/CIFAR10-LP-Label-Noise/fig.tex <==
% \setlength{\abovecaptionskip}{2pt}  % Set this globally just after loading your packages
% \setlength{\intextsep}{-1pt}         % Reduce space above and below the floats
\begin{figure} 
\centering
\subfloat[\textsc{No Corruption}]
{\includegraphics[width=0.32\textwidth]{plots/CIFAR10-LP-Label-Noise/psi=0.png}}
\subfloat[\textsc{20\% Symm Label Noise}]
{\includegraphics[width=0.32\textwidth]{plots/CIFAR10-LP-Label-Noise/psi=20.png}}
\subfloat[\textsc{40\% Symm Label Noise}]
{\includegraphics[width=0.32\textwidth]{plots/CIFAR10-LP-Label-Noise/psi=40.png}}
\label{fig:CIFAR10-LP-Label-Noise}
\caption{CIFAR10 Linear Probing over ResNet-18 (proxy) pretrained on ImgageNet-1k}
\end{figure}

==> plots/CIFAR10-LP-Label-Noise/main-fig.tex <==
% \setlength{\abovecaptionskip}{2pt}  % Set this globally just after loading your packages
% \setlength{\intextsep}{-1pt}         % Reduce space above and below the floats
\begin{figure*}[t]
\centering
\subfloat[\textsc{No Corruption}]
{\includegraphics[width=0.3\textwidth]{plots/CIFAR10-LP-Label-Noise/psi=0.png}}
\subfloat[\textsc{20\% Symm Label Noise}]
{\includegraphics[width=0.3\textwidth]{plots/CIFAR10-LP-Label-Noise/psi=20.png}}
\subfloat[\textsc{40\% Symm Label Noise}]
{\includegraphics[width=0.3\textwidth]{plots/CIFAR10-LP-Label-Noise/psi=40.png}}

\caption{
\footnotesize
{\bf Domain Transfer ( ImageNet-1k $\rightarrow$ CIFAR-10 ) Proxy + Embedding :} We train a Linear Classifier on CIFAR10; over embeddings obtained from a frozen ResNet-18 pretrained on ImageNet-1k. The dataset was pruned using the same encoder.
We compare our method $\gmm$ with geometric pruning baselines: \textsc{Uniform}, \textsc{Easy},\textsc{Hard}, \textsc{Moderate}, \textsc{Herding} across different label noise settings.
}
\label{fig:main-cifar-lp}
\end{figure*}

==> plots/corruption_demo/fig.corr_demo.tex <==
\begin{figure}[t]
\centering
%\setlength{\abovecaptionskip}{0pt} 
\subfloat[\textsc{Original}]
{\includegraphics[width=0.24\textwidth]{plots/corruption_demo/demo.pdf}}
\subfloat[\textsc{50\% pixel-Corr}]
{\includegraphics[width=0.24\textwidth]{plots/corruption_demo/demo_c=50.pdf}}
\subfloat[\textsc{70\% pixel-Corr}]
{\includegraphics[width=0.24\textwidth]{plots/corruption_demo/demo_c=70.pdf}}
\subfloat[\textsc{90\% pixel-Corr}]
{\includegraphics[width=0.24\textwidth]{plots/corruption_demo/demo_c=90.pdf}}
\label{fig:demo-img-corr}
\end{figure}

==> plots/toy/fig.toy-all.tex <==
\begin{figure} 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[Uniform ($\psi=0$)]{
\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/uniform.png}}
\subfloat[Uniform ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/uniform.png}}
\subfloat[Uniform ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/uniform.png}}
\\
\subfloat[Easy ($\psi=0$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/easy.png}}
\subfloat[Easy ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/easy.png}}
\subfloat[Easy ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/easy.png}}
\\
\subfloat[Hard ($\psi=0$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/hard.png}}
\subfloat[Hard ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/hard.png}}
\subfloat[Hard ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/hard.png}}
\\
\subfloat[Moderate ($\psi=0$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/moderate.png}}
\subfloat[Moderate ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/moderate.png}}
\subfloat[Moderate ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/moderate.png}}
\\
\subfloat[Herding ($\psi=0$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/herding.png}}
\subfloat[Herding ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/herding.png}}
\subfloat[Herding ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/herding.png}}
\\
\subfloat[Robust Herding ($\psi=0$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=0/robust-herding.png}}
\subfloat[Robust Herding ($\psi=0.2$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=20/robust-herding.png}}
\subfloat[Robust Herding ($\psi=0.45$)]
{\includegraphics[width=0.25\textwidth]{plots/toy/corr=45/robust-herding.png}}
\caption{\footnotesize Toy Example.}

\label{fig:toy-allcorr=45}
\end{figure}

==> plots/toy/fig.toy-corr=0.tex <==
% \setlength{\abovecaptionskip}{2pt}  % Set this globally just after loading your packages
% \setlength{\intextsep}{-1pt}         % Reduce space above and below the floats
\begin{figure*} 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[\textsc{Uniform}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=0/uniform.png}}
\subfloat[\textsc{Easy}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=0/easy.png}}
\subfloat[\textsc{Hard}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=0/hard.png}}
\\
\subfloat[\textsc{Moderate}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=0/moderate.png}}
\subfloat[\textsc{Herding}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=0/herding.png}}
\subfloat[$\gm$ \textsc{Matching}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=0/robust-herding.png}}
\caption{\footnotesize {\bf No Corruption :} We select 10\% of the samples using: (\textsc{Uniform}) Random Sampling, (\textsc{Easy}) Selection of samples closest to the centroid. (\textsc{Hard}) Selection of samples farthest from the centroid. (\textsc{Moderate}) Selection of samples closest to the median distance from the centroid. (\textsc{Herding}) Moment Matching, (\textsc{GM Matching}) Robust Moment (GM) Matching~\eqref{eq:gm_matching}.}

\label{fig:toy-corr=0}
\end{figure*}

==> plots/toy/fig.toy-corr=20.tex <==
% \setlength{\abovecaptionskip}{2pt}  % Set this globally just after loading your packages
% \setlength{\intextsep}{-1pt}         % Reduce space above and below the floats
\begin{figure*}[t]
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[\textsc{Uniform}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=20/uniform.png}}
\subfloat[\textsc{Easy}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=20/easy.png}}
\subfloat[\textsc{Hard}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=20/hard.png}}
\\
\subfloat[\textsc{Moderate}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=20/moderate.png}}
\subfloat[\textsc{Herding}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=20/herding.png}}
\subfloat[$\gm$ \textsc{Matching}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=20/robust-herding.png}}
\caption{\footnotesize {\bf 20\% Corruption}: In this experiment, 20\% of the samples are corrupted -- drawn from a adversary chosen distribution (red). We select 10\% samples using: (\textsc{Uniform}) Random Sampling, (\textsc{Easy}) Selection of samples closest to the centroid. (\textsc{Hard}) Selection of samples farthest from the centroid. (\textsc{Moderate}) Selection of samples closest to the median distance from the centroid. (\textsc{Herding}) Moment Matching, (\textsc{GM Matching}) Robust Moment (GM) Matching~\eqref{eq:gm_matching}. We see that while \textsc{Easy} remains robust, it is clearly sampling from low-density areas -- failing to capture the prototypical samples.}
\label{fig:toy-corr=20}
\end{figure*}

==> plots/toy/fig.toy-corr=40.tex <==
% \setlength{\abovecaptionskip}{2pt}  % Set this globally just after loading your packages
% \setlength{\intextsep}{-1pt}         % Reduce space above and below the floats
\begin{figure*} 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[\textsc{Uniform}]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=40/uniform.png}}
\subfloat[\textsc{Easy}]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=40/easy.png}}
\subfloat[\textsc{Hard}]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=40/hard.png}}
\\
\subfloat[\textsc{Moderate}]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=40/moderate.png}}
\subfloat[\textsc{Herding}]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=40/herding.png}}
\subfloat[$\gm$ \textsc{Matching}]
{\includegraphics[width=0.3\textwidth]{plots/toy/corr=40/robust-herding.png}}
\caption{\footnotesize {\bf \textsc{Data Pruning in The Wild}}: 
Data Pruning methods applied to samples from a multivariate Gaussian distribution (blue), with 40\% replaced by an adversarial distribution (red). We subset 10\% of the examples using: (\textsc{Uniform}) Random Sampling, (\textsc{Easy}) Selection of samples closest to the centroid. (\textsc{Hard}) Selection of samples farthest from the centroid. (\textsc{Moderate}) Selection of samples closest to the median distance from the centroid. (\textsc{Herding}) Moment Matching, (\textsc{GM Matching}) Robust Moment (GM) Matching~\eqref{eq:gm_matching}. $\gmm$ yields significantly more robust (from the true distribution) subset than the other approaches.}

\label{fig:toy-corr=40}
\end{figure*}

==> plots/toy/fig.toy-corr=45.tex <==
% \setlength{\abovecaptionskip}{2pt}  % Set this globally just after loading your packages
% \setlength{\intextsep}{-1pt}         % Reduce space above and below the floats
\begin{figure*}[t] 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[\textsc{Uniform}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=45/uniform.png}}
\subfloat[\textsc{Easy}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=45/easy.png}}
\subfloat[\textsc{Hard}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=45/hard.png}}
\\
\subfloat[\textsc{Moderate}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=45/moderate.png}}
\subfloat[\textsc{Herding}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=45/herding.png}}
\subfloat[$\gm$ \textsc{Matching}]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=45/robust-herding.png}}
\caption{\footnotesize {\bf Toy Example:} {\bf 45\% of the samples are corrupted} i.e. drawn from an adversary chosen distribution (red). We compare several baselines for choosing 10\% samples: (\textsc{Uniform}) random sampling, (\textsc{Easy}) selects of samples closest to the centroid. (\textsc{Hard}) Selection of samples farthest from the centroid. (\textsc{Moderate}) selects samples closest to the median distance from the centroid. (\textsc{Herding}) moment matching, (\textsc{GM Matching}) robust moment (GM) matching~\eqref{eq:gm_matching}. Clearly $\gm$ Matching is significantly more robust and diverse than the other approaches even at such high corruption rates.}

\label{fig:toy-corr=45}
\end{figure*}

==> plots/toy/fig.toy-mean-est-2.tex <==
\begin{figure*} 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[No Corruption]{
\includegraphics[width=0.32\textwidth]{plots/toy/gm-viz/corruption_0.png}}
\subfloat[30\% Corruption]
{\includegraphics[width=0.32\textwidth]{plots/toy/gm-viz/corruption_0.3.png}}
\subfloat[50\% Corruption]
{\includegraphics[width=0.32\textwidth]{plots/toy/gm-viz/corruption_0.5.png}}

\caption{\footnotesize {\bf \textsc{Robust Mean Estimation}}: As the corruption rate $0 \leq \psi < \frac{1}{2}$ increases ( representing the fraction of samples drawn from an adversary-chosen distribution), the empirical mean increasingly deviates from the true uncorrupted mean. In contrast, the geometric median ($\gm$) remains robust and stays closer to the uncorrupted (oracle) mean, demonstrating its resilience to outliers and corrupted data.}
\label{fig:toy-mean-estimation-2}
\end{figure*}

==> plots/toy/fig.toy_mean-estimation.tex <==
\begin{figure*} 
\centering
% \setlength{\abovecaptionskip}{0pt} 
\subfloat[$\psi = 0$]{
\includegraphics[width=0.32\textwidth]{plots/toy/corr=0/dist.png}}
\subfloat[$\psi = 0.2$]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=20/dist.png}}
\subfloat[$\psi = 0.45$]
{\includegraphics[width=0.32\textwidth]{plots/toy/corr=45/dist.png}}

\caption{\footnotesize {\bf \textsc{Robust Mean Estimation}}: As we progressively increase $0 \leq \psi < 1/2$ (fraction of corrupt samples in the data); while the empirical mean drifts away,  $\gm$ remains close to the uncorrupted mean.}
\label{fig:toy-mean-estimation}
\end{figure*}



==> workshop_fmwild.tex <==
\usepackage{icml_fmwild}
\newcommand{\gm}{\textsc{Gm}}
\newcommand{\gmm}{\textsc{Gm Matching}}
\newcommand{\Mu}{\bm{\mu}}

% to compile a camera-ready version, add the [final] option, e.g.:
%     \usepackage[final]{neurips_2024}

\setlength{\parindent}{0pt}
\setlength{\parskip}{5 pt}
\setlength{\fboxsep}{5pt} % Adjust the spacing between the text and the box outline
\setlength{\fboxrule}{1pt} % Adjust the thickness of the box outline

\input{defpack}
\PassOptionsToPackage{cmyk}{xcolor}
\begin{document}


\end{document}
